Tracking in Order to Recover: Detectable Recovery of Lock-Free Data Structures

This paper presents the tracking approach for deriving detectably recoverable (and thus also durable) implementations of many widely-used concurrent data structures. Such data structures, satisfying detectable recovery, are appealing for emerging systems featuring byte-addressable non-volatile main memory (NVRAM), whose persistence allows to efficiently resurrect failed processes after crashes. Detectable recovery ensures that after a crash, every executed operation is able to recover and return a correct response, and that the state of the data structure is not corrupted. Info-Structure Based (ISB)-tracking amends descriptor objects used in existing lock-free helping schemes with additional fields that track an operation's progress towards completion and persists these fields to memory in order to ensure detectable recovery. ISB-tracking avoids full-fledged logging and tracks the progress of concurrent operations in a per-process manner, thus reducing the cost of ensuring detectable recovery. We have applied ISB-tracking to derive detectably recoverable implementations of a queue, a linked list, a binary search tree, and an exchanger. Experimental results show the feasibility of the technique.

==> code-BST-Delete.tex <==

%\newgeometry{top=0.5in, left=0.75in, right=0.75in}

%\begin{figure*}[!t]
	
	\begin{algorithm}[hp]

		\removelatexerror
		\scriptsize
		\begin{flushleft}	
		\end{flushleft}
%		\vspace{-5mm}
		
%%%%%%%%%%%%%%%%%%%%%%%%%%%% DELETE FUNCTION %%%%%%%%%%%%%%%%%%%%%%%%%%%

			\begin{procedure}[H]
				\caption{() \small boolean \func{Delete} ($\Key\ k$)}
				
				Internal *$gp$, *$p$ \label{BST-delete-entry} \;
				Leaf *$l$ \;
				Update $pupdate, gpupdate, result$ \;
				\DFlag\ *$op$ \;
				\textcolor{blue} {$RD_q$ := \init} \label{BST-delete-reset-RD} \;
				\textcolor{blue} {$\text{CP}_q := 1$}  \tcp*{set a check-point indicating \DFlag} \label{BST-delete-set-checkpoint}
														\nonl \hspace*{17mm}\tcp{structure was installed}				
				\While {\True \label{BST-delete-while-loop}} {
					$\langle gp, p, l, pupdate, gpupdate \rangle := \func{Search}(k)$ \label{BST-delete-search} \;
					\uIf (\tcp*[f]{key $k$ is not in the tree}) {$l. key \neq k$ \label{BST-delete-if-false}} {
						\textcolor{blue} {$RD_q :=$ pointer to a new \DFlag\ \record\ containing $\langle \init, \init, \init, \False \rangle$} \tcp*{persist response} \label{BST-delete-persist-false}
						\KwRet \False \label{BST-delete-return-false}
					}
					\tcp{help the other operation (if any)}
					\lIf {$gpupdate.state \neq \clean$} {\func{Help}$(gpupdate)$} \label{BST-delete-help-gp}
					\tcp{help the other operation (if any)}					
					\lElseIf {$pupdate.state \neq \clean$} {\func{Help}$(pupdate)$} \label{BST-delete-help-p}
					\uElse {
						$op :=$ pointer to a new \DFlag\ \record\ containing \;
						\nonl \hspace*{3mm} $\langle gp, p, l, pupdate, \textcolor{blue}{\init} \rangle$ \label{BST-delete-new-DFlag} \;
						\tcp{update info-structure for current attempt}
						\textcolor{blue}{$RD_p := op$}  \label{BST-delete-update-RD} \;
						\tcp{\bf dflag \CAS}
						$result := gp. update. \CAS\ (gpupdate, \langle \deleteflag, op \rangle)$  \label{BST-delete-dflag-cas} \;
						\uIf {$result = gpupdate$ \label{BST-delete-if-dflag}} {
							\tcp{the dflag \CAS\ was successful, so either}
							\tcp{finish deletion or unflag}
							\lIf {\func{HelpDelete}$(op)$} {\KwRet \True} \label{BST-delete-return-true}
						}
						\lElse (\tcp*[f]{the dflag \CAS\ failed; help the operation that caused the failure}) {\func{Help}$(result)$} \label{BST-delete-help-after-failure}
					}
				}
			\end{procedure}
		
%%%%%%%%%%%%%%%%%%%%%%%%%%%% HELP-DELETE FUNCTION %%%%%%%%%%%%%%%%%%%%%%

			\begin{procedure}[H]
				\caption{() \small boolean \func{HelpDelete} (\DFlag\ *$op$)}
				
				% \nonl \com {\it Precondition}:  $op$ points to a \DFlag\ \record\  (\ie, it is not \NULL) \;
				Update $result$ \;
				\tcp{\bf mark \CAS}
				$result := op. p. update. \CAS\ (op. pupdate, \langle \mk, op\rangle)$  \label{BST-helpDelete-mark-cas}\;
				\uIf {$result = op. pupdate$ or $result = \langle \mk, op\rangle$ \label{BST-helpDelete-if-marked}} {
					\tcp{$op. p$ is successfully marked}
					\func{HelpMarked}$(op)$ \tcp*{complete the deletion} \label{BST-helpDelete-call-helpMarked}
					\KwRet \True \label{BST-helpDelete-return-true}
				}
				\uElse (\tcp*[f]{the mark \CAS\ failed}) {
					\func{Help}$(result)$ \tcp*{help operation that caused failure} \label{BST-helpDelete-help-after-failure}
					$op. gp. update. \CAS\ (\langle \deleteflag, op\rangle, \langle \clean, op\rangle)$ \tcp*{\bf backtrack \CAS} \label{BST-helpDelete-backtrack-cas}
					\KwRet \False \tcp*{delete attempt failed} \label{BST-helpDelete-return-false}
				}
			\end{procedure}
		
%%%%%%%%%%%%%%%%%%%%%%%%%%%% HELP-MARKED FUNCTION %%%%%%%%%%%%%%%%%%%%%%%%

			\begin{procedure}[H]
				\caption{() \small boolean \func{HelpMarked} (\DFlag\ *$op$)}
				
				% \nonl \com {\it Precondition}:  $op$ points to a \DFlag\ \record\  (\ie, it is not $\NULL$) \;
				Node *$other$ \;
				\nonl \com Set $other$ to point to the sibling of the node to which  $op. l$ points \;
				\leIf {$op. p. right = op. l$} {$other := op. p. \lft$} {$other:=op. p. right$} \label{BST-helpMarked-set-other}
				\nonl \com Splice the node to which $op. p$ points out of the tree, replacing it by $other$ \;
				\func{CAS-Child}$(op. gp, op. p, other)$ \tcp*{\bf dchild \CAS} \label{BST-helpMarked-dchild-cas}
				\textcolor{blue}{$op.result := \True$} \tcp*{announce the operation completed} \label{BST-helpMarked-set-result}
				$op. gp. update. \CAS\ (\langle \deleteflag, op\rangle, \langle \clean, op\rangle)$ \tcp*{\bf dunflag \CAS} \label{BST-helpMarked-dunflag-cas}
			\end{procedure}
		
%%%%%%%%%%%%%%%%%%%%%%%%%%%% HELP FUNCTION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		
		\begin{procedure}[H]
			\caption{() \small \func{Help} (Update $u$)}
			
			\nonl \com General-purpose helping routine \;
			% \nonl \com {\it Precondition}:  $u$ has been stored in the $update$ field of some internal node \;
			\lIf {$u.state = \insertflag$} {\func{HelpInsert}$(u.\info)$} \label{BST-help-call-HelpInsert}
			\lElseIf {$u.state = \mk$} {\func{HelpMarked}$(u.\info)$} \label{BST-help-call-HelpMarked}
			\lElseIf {$u.state = \deleteflag$} {\func{HelpDelete}$(u.\info)$} \label{BST-help-call-HelpDelete}
		\end{procedure}
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%% CAS-CHILD FUNCTION %%%%%%%%%%%%%%%%%%%%%%%%%
	
		\begin{procedure}[H]
			\caption{() \small \func{CAS-Child} (Internal *$parent$, Node *$old$, Node *$new$)} \label{CAS-Child}
			
			% \nonl \com {\it Precondition}:  $parent$ points to an Internal node and $new$ points to a Node (\ie, neither is \NULL) \;
			\nonl \com This routine tries to change one of the child fields of the node that $parent$ points to from $old$ to $new$. \;
			\uIf {$new. key < parent. key$ \label{which-child}} {
				$parent. \lft. \CAS\ (old, new)$ \label{BST-casChild-left-cas}
			}
			\uElse {
				$parent. right. \CAS\ (old, new)$ \label{BST-casChild-right-cas}
			}
		\end{procedure}
			
		\caption{Recoverable BST: \func{Delete} \& auxiliary routines.}
		\label{BST-code3}
	\end{algorithm}
	
%\end{figure*}

%\restoregeometry


==> code-BST-Insert.tex <==

%\newgeometry{top=0.5in, left=0.75in, right=0.75in}

%\begin{figure*}[!t]
	
	\begin{algorithm}[hp]
		\removelatexerror
		\scriptsize
		\begin{flushleft}	
		\end{flushleft}
%		\vspace{-5mm}
		
%%%%%%%%%%%%%%%%%%%%%%%%%%%% SEARCH FUNCTION %%%%%%%%%%%%%%%%%%%%%%%%%%
		
		\begin{procedure}[H]
			\caption{() \small $\langle \mbox{Internal*}, \mbox{Internal*}, \mbox{Leaf*}, \mbox{Update}, \mbox{Update}\rangle$ \func{Search} ($\Key\ k$)}
			
			\nonl \com Used by \func{Insert}, \func{Delete} and \func{Find} to traverse a branch of the BST; satisfies following {\it postconditions}: \;
			\nonl \com \hspace*{2mm} \postnotnull\ $l$ points to a Leaf node and $p$ points to an Internal node \;
			\nonl \com \hspace*{2mm} \postl\ Either $p. \lft$ has contained $l$ (if $k<p. key$) or $p. right$\; 
			\nonl \com \hspace*{5mm} has contained $l$ (if $k\geq p. key$) \;
			\nonl \com \hspace*{2mm} \postpup\ $p. update$ has contained $pupdate$ \;
			\nonl \com \hspace*{2mm} \postnonempty\ if $l. key\neq \infty_1$, then the following three statements hold: \;
			\nonl \com \hspace*{5mm}\postgpnotnull\ $gp$ points to an Internal node\ \;
			\nonl \com \hspace*{5mm}\postp\ either $gp. \lft$ has contained $p$ (if $k<gp. key$) or $gp.right$ \; 
			\nonl \com \hspace*{9mm} has contained $p$ (if $k\geq gp. key$) \;
			\nonl \com \hspace*{5mm}\postgpup\ $gp. update$ has contained $gpupdate$ \;
			
			Internal *$gp$, *$p$ \;
			Node *$l:= Root$  \label{restart-search} \;
			Update $gpupdate, pupdate$ \tcp*{each stores a copy of an} 
			\nonl \hspace*{29mm} \tcp{$update$ field}

			\While {$l$ points to an internal node \label{BST-search-while-loop}} {
				$gp := p$ \tcp*{remember parent of $p$} \label{BST-search-set-gp}
				$p := l$ \tcp*{remember parent of $l$} \label{BST-search-set-p}
				$gpupdate := pupdate$ \tcp*{remember $update$ field of $gp$} \label{BST-search-set-gpupdate}
				$pupdate := p. update$ \tcp*{remember $update$ field of $p$} \label{BST-search-set-pupdate}
				\tcp*{move down to appropriate child}
				\leIf {$k < l. key$} {$l:= p. \lft$} {$l:=p. right$} \label{BST-search-read-child}
			}
			\KwRet $\langle gp, p, l, pupdate, gpupdate \rangle$ \label{BST-search-return}

		\end{procedure}
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%% FIND FUNCTION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

		\begin{procedure}[H]
			\caption{() \small Leaf* \func{Find} ($\Key\ k$)}
			
			Leaf *$l$ \;
			$\langle -,-,l,-,-\rangle := \func{Search}(k)$ \label{BST-find-call-search} \;
			\lIf {$l. key = k$} {\KwRet $l$} \label{BST-find-return-l}
			\lElse {\KwRet \NULL} \label{BST-find-return-null}
		\end{procedure}
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%% INSERT FUNCTION %%%%%%%%%%%%%%%%%%%%%%%%%%%%

		\begin{procedure}[H]
			\caption{() \small boolean \func{Insert} ($\Key\ k$)}
			
			Internal *$p$, *$newInternal$ \label{BST-Insert-entry} \;
			Leaf *$l$, *$newSibling$ \;
			Leaf *$new :=$ pointer to a new Leaf node whose $key$ field is $k$ \label{BST-insert-create-leaf} \;
			Update $pupdate, result$ \;
			\IFlag\ *$op$ \;
			
			\textcolor{blue} {$RD_q$ := \init} \label{BST-insert-reset-RD} \;
			\textcolor{blue} {$\text{CP}_q := 1$}  \tcp*{set a check-point indicating \IFlag} \label{BST-insert-set-checkpoint}
												   \nonl \hspace*{17mm}\tcp{structure was installed}
			\While {\True \label{BST-insert-while-loop}} {
				$\langle -, p, l, pupdate, - \rangle := \func{Search}(k)$ \label{BST-insert-search} \;
				\uIf (\tcp*[f]{cannot insert duplicate key}) {$l. key = k$ \label{BST-insert-if-false}} {
					\tcp{persist response}					
					\textcolor{blue} {$RD_q :=$ pointer to a new \IFlag\ \record\ containing $\langle \init, \init, \init, \False \rangle$} \label{BST-insert-persist-false} \;
					\KwRet \False \label{BST-insert-return-false}
				}
				\tcp{help the other operation}
				\lIf {$pupdate.state \neq \clean$} {\func{Help}$(pupdate)$} \label{BST-insert-help-unclean}
				\uElse {
					\tcp{make a duplicate of $l$}
					$newSibling :=$ pointer to a new Leaf whose key is $l. key$ \label{BST-insert-create-sinling}\;
					$newInternal :=$ pointer to a new Internal node with $key$ field \;
					\nonl \hspace*{12mm} $\max(k, l. key)$, $update$ field $\langle \clean, \NULL\rangle$, and \label{BST-insert-create-internal} \;
					\nonl \hspace*{12mm}  with two child fields equal to $new$ and $newSibling$ \;
					\nonl \hspace*{12mm} (the one with the smaller key is the left child) \;
					$op :=$ pointer to a new \IFlag\ \record\  containing \;
					\nonl \hspace*{5mm} $\langle p, l, newInternal, \textcolor{blue}{\init} \rangle$ \label{BST-insert-new-IFlag} \;
					\tcp{update info-structure for current attempt}
					\textcolor{blue}{$RD_q := op$} \label{BST-insert-update-RD} \;
					$result := p. update. \CAS\ (pupdate, \langle \insertflag, op\rangle)$ \tcp*{\bf iflag \CAS} \label{BST-insert-iflag-cas}
					\uIf (\tcp*[f]{the iflag \CAS\ succeeded}) {$result = pupdate$ \label{BST-insert-if-iflag}} {
						\func{HelpInsert}$(op)$ \tcp*{finish the insertion} \label{BST-insert-finish-insert}
						\KwRet \True\ \label{BST-insert-return-true} \;
					}
					\lElse (\tcp*[f]{the iflag \CAS\ failed; help the operation that caused failure}) {\func{Help}$(result)$} \label{BST-insert-help-after-failure}
				}
			}
		\end{procedure}
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%% HELP-INSERT FUNCTION %%%%%%%%%%%%%%%%%%%%%

		\begin{procedure}[H]
			\caption{() \small \func{HelpInsert} (\IFlag\ *$op$)}
			
			% \nonl \com {\it Precondition}:  $op$ points to an \IFlag\ \record\  (\ie, it is not $\NULL$) \;
			\func{CAS-Child}$(op. p, op. l, op. newInternal)$ \tcp*{\bf ichild \CAS} \label{ichild-cas} \label{BST-helpInsert-cas-child}
			\textcolor{blue}{$op.result := \True$} \tcp*{announce the operation completed} \label{BST-helpInsert-set-result}
			$op. p. update. \CAS\ (\langle \insertflag, op \rangle, \langle \clean, op\rangle)$ \tcp*{\bf iunflag \CAS} \label{BST-helpInsert-iunflag-cas}
		\end{procedure}
			
		\caption{Recoverable BST: \func{Search}, \func{Find}, \func{Insert}}
		\label{BST-code2}
	\end{algorithm}
	
%\end{figure*}

%\restoregeometry


==> code-DT-linked-list.tex <==

\SetKwRepeat{Do}{do}{while}


%	\hspace*{-0.3in}
	\begin{algorithm}[!t]
		
		
	%	\begin{multicols*}{2}
		\removelatexerror
		\scriptsize
			
		\begin{flushleft}
			
			\begin{tabular}{ll}
				\textbf{Type} Node & \{MarkableNodeRef $next$, int \emph{key}, \textcolor{blue} {int \emph{deleter}}\} \\
				\textcolor{blue}{\textbf{Type} \Info} & \textcolor{blue} {\{Node $nd$, boolean $result$\}} \\
			\end{tabular}
		
			\textbf{Shared variables:} Node $head$ \\
			\textbf{Private variables:} \textcolor{blue} {$\Info\ RD_p$ for each process p}
		\end{flushleft}	
			
		
		%%%%%%%%%%%%%%%%%%%%%% Linked List - Find %%%%%%%%%%%%%%%%%%%%%%%%
		\begin{procedure}[H]
			\caption{() \small Boolean \find\ (T $key$)}
			
			$\langle pred, curr \rangle := \search (key)$ \label{ll-find-start} \;
			\lIf {$curr.key \neq key$} {
				\KwRet \False	
			}
			\lElse {\KwRet \True} \label{ll-find-end}
		\end{procedure}
	
	
		%%%%%%%%%%%%% Recoverable Linked List - Delete %%%%%%%%%%%%%%%%%%%
		
		\begin{procedure}[H]
			\caption{() \small Boolean \delete\ (T $key$)}
			
			Node $pred$, $curr$, $succ$  \;
			boolean $res$ := \False \;
			\textcolor{blue} {$RD_p$ := \textbf{new} \Info\ (\init, \init) \tcp*{set \Info\ structure}} \label{ll-delete-persist-to-RDp}
			\textcolor{blue} {$CP_p := 1$ \tcp*{set a check-point} \label{ll-delete-set-checkpoint}}
			
			\While {\True} {
				$\langle pred, curr \rangle := \search (key)$ \tcp*{search for $key$} \label{ll-search-in-delete}
				\uIf (\tcp*[f]{$key$ not in the list}) {$curr.key \neq key$ \label{ll-delete-key-in-list}} {
					\textcolor{blue} {$RD_p.result := \False$ \tcp*{persist response}} \label{ll-delete-write-false}
					\KwRet \False \label{ll-delete-return-false}
				}
				\uElse {
					\textcolor{blue}{$RD_p.nd := curr$ \tcp*{persist curr reference}} \label{ll-delete-update-nd}
					$succ := curr.next$ \label{ll-delete-set-succ-to-next}\;
					\uIf {\CAS ($curr.next$, $unmark(succ)$, $mark(succ)$) \label{ll-delete-logical-delete}} {
						\textbf{break} \;
					}
				}
			}
			%$succ := curr.next$ \label{ll-delete-read-succ-after-CAS}\;
			\uIf {\CAS ($pred.next$, $curr$, $unmark(succ)$) \label{ll-delete-physical-delete1}}{
				$\search (key)$ \tcp*{Physical deletion} \label{ll-delete-physical-delete2}
			}
			\textcolor{blue}{\tcp{try establishing yourself as deleter}}
			\textcolor{blue}{$res := \CAS (curr.deleter, \init, p)$}  \label{ll-delete-CAS-deleter} \;
			\textcolor{blue}{$RD_p.result := res$ \tcp*{persist response}} \label{ll-delete-write-after-CAS}
			\KwRet $res$ \label{ll-delete-return-res}
		
			\remove{
					\While {$\lnot ismarked(curr.next)$  \label{ll-delete-while-loop}}{
						\tcp{repeatedly attempt logical delete}
						$succ := curr.next$ \label{ll-delete-set-succ-to-next}\;
					}
					\tcp{Physical deletion attempt}
					$succ := curr.next$ \label{ll-delete-read-succ-after-CAS}\;
					\CAS ($pred.next$, $curr$, $unmark(succ)$) \label{ll-delete-physical-delete} \;
				}
		\end{procedure}
	
		%%%%%%%%%%%%%% Recoverable Linked List - Insert %%%%%%%%%%%%%%%%%
		
		\begin{procedure}[H]
			\caption{() \small Boolean \insertlst\ (T $key$)}
			
			Node $pred$, $curr$, $newnd$ := \textbf{new} Node ($\init, key, \textcolor{blue}{\init}$) \label{ll-insert-entry} \;
			%Node $newnd$ := \textbf{new} Node ($\init, key, \textcolor{blue}{\init}$)\;
			%\textcolor{blue}{newnd.deleter := \init} \;
			\textcolor{blue} {$RD_p$ := \textbf{new} \Info\ ($newnd$, \init) \label{ll-insert-install-IS}} \;
			\textcolor{blue} {$\text{CP}_p := 1$ \tcp*{set a check-point}\label{ll-insert-set-checkpoint}}
			\While{\True}{ \label{ll-insert-while}
				\tcp{search for right location to insert}
				$\langle pred, curr \rangle := \search(key)$ \label{ll-insert-search} \;
				\uIf (\tcp*[f]{$key$ in the list}) {$curr.key = key$ \label{ll-insert-if-in-list}} {
					\textcolor{blue} {$RD_p.result := \False$ \tcp*{persist response} \label{ll-insert-persist-false-response}}
					\KwRet \False \label{ll-insert-return-false}
				} \uElse {
					$newnd.next$ := $curr$\;
					\uIf (\tcp*[f]{try adding newnd}) {\CAS ($pred.next$, $curr$, $newnd$) \label{ll-insert-CAS}} {
						\textcolor{blue} {$RD_p.result := \True$ \label{ll-insert-persist-true-response}} \;
						\KwRet \True
					}
				}		
			}
		\end{procedure}
		
		\caption{Direct-Tracking Linked List: \find, \insertlst\ \& \delete\ (code for process $p$)}
		\label{alg:direct-tracking-ll-1}
	\end{algorithm}


	\begin{algorithm}
		\nonl
		\removelatexerror
		\scriptsize
		%\begin{flushleft}
		%\end{flushleft}	
	
		%%%%%%%%%%%%%%%%%%%%%% Linked List - Search %%%%%%%%%%%%%%%%%%%%%%%%
		
		\begin{procedure}[H]
			\caption{() \small $\langle$Node, Node$\rangle$ \search\ (T $key$)}
			
			Node $pred$, $curr$, $succ$, $pred\_next$ \;
			
			\While{\True}{
				$curr := head$ \;
				$succ := head.next$ \;
				\Do {$ismarked(succ)$ or $curr.key < key$} {
					\uIf {$ismarked(succ) = \False$} {
						$pred := curr$ \;
						$pred\_next := curr.next$ \;
					}
					$curr := unmark(succ)$ \;
					$succ := curr.next$ \;
				}
				\uIf {$pred\_next = curr$} {
					\uIf {$ismarked(curr.next) = \False$} {
						\KwRet $\langle pred, curr \rangle$ \;	
					}	
				}
				\uIf {$\CAS (pred.next, pred\_next, curr)$} {
					\uIf {$ismarked(curr.next) = \False$} {
						\KwRet $\langle pred, curr \rangle$ \;	
					}	
				}
			}
		\remove{
				\hspace*{5mm} $curr := pred.next$ \label{ll-search-read-cur}\;	
				\While{\True}{
					$succ := curr.next$ \;
					\tcp{if $curr$ was logically deleted}
					\uIf {$ismarked(succ)$} {
						\uIf (\tcp*[f]{help delete}) {$\CAS (pred.next, curr$, $unmark(succ)$) = \False}{
							\textbf{go to} retry \tcp*{help failed}
						}
						$curr := unmark(succ)$ \tcp*{help succeeded}
					} \uElse {
						\uIf (\tcp*[f]{first unmarked node with key $\geq key$}) {$curr.key \geq key$} {
							\KwRet $\langle pred,curr \rangle$
						}
						$pred := curr$ \tcp*{advance $pred$}
						$curr := succ$ \tcp*{advance $curr$}
					}
				}
			}
		\end{procedure}
	
	
	%%%%%%%%%%%%% Recoverable Linked List - Delete Recover %%%%%%%%%%%%
	
		\begin{procedure}[H]
			\color{blue}{
			\caption{() \small \text{Boolean \deleterecover\ (T $key$)}}
			Node $nd$ := $RD_p.nd$ \;
			boolean $res$ := \False \;
			\uIf {$CP_p = 0$ \label{ll-delete-recover-read-CP}} {
				\tcc{failed before check-point}
				Re-invoke \delete
			}
			\uIf {$RD_p.result \neq \init$ \label{ll-delete-recover-response-persisted}} {
				\tcc{operation response was persisted}
				\KwRet $RD_p.result$ \label{ll-delete-recover-return-persisted-response}
			}
			\uIf {$nd \neq \init$ \&\& $ismarked(nd.next)$ \label{ll-delete-recover-if-should-perform-deleter-CAS}} {
				\tcc{$nd$ was logically deleted; try establish yourself as deleter}
				$\CAS (nd.deleter, \init, p)$ \label{ll-delete-recover-deleter-CAS} \;
				$res := (nd.deleter == p)$ \label{ll-delete-recover-read-deleter} \;
				$RD_p.result := res$ \tcp*{persist response}
				\KwRet res \label{ll-delete-recover-return-res}\;
			}
			\lElse {
				Re-invoke \delete \label{ll-delete-recover-reattempt-deletion} \tcp*[f]{re-attempt deletion}
			}
		}
		\end{procedure}
	
	%%%%%%%%%%%%% Recoverable Linked List - Insert Recover %%%%%%%%%%
	
		\begin{procedure}[H]
			\color{blue} {
			\caption{() \small \text{Boolean \insertrecover\ (T $key$)}}
			%
			Node $nd := RD_p.nd$\;
			\uIf {$CP_p := 0$ \label{ll-insert-recover-read-CP}} {
				\tcc{failed before check-point}		
				Re-invoke \insertlst \label{ll-insert-recover-re-invoke}
			}
			\uIf {$RD_p.result \neq \init$ \label{ll-insert-recover-response-persisted}} {
				\tcc{operation response was persisted}
				\KwRet $RD_p.result$ \tcp*[f]{return response \label{ll-insert-recover-return-persisted-response}}
			}
			$\langle pred, curr \rangle := \search (key)$ \label{ll-insert-recover-search} \;
			\uIf {$curr = nd \mid \mid ismarked(nd.next)$ \label{ll-insert-if-was-linearized}} {
				\tcp{$nd$ in list or is marked (hence was)}
				$RD_p.result := \True$ \tcp*{persist response} \label{ll-insert-linearized-persist-true}
				\KwRet \True \label{ll-insert-linearized-return-true}\;
			}
			\lElse
			{
				Re-invoke \insertlst \tcp*[f]{re-attempt insertion}
			}
		}
		\end{procedure}
	
	%\end{multicols*}
		
		\caption{Direct-Tracking Linked List: \search\ and \recover\ functions (code for process $p$)}
		\label{alg:direct-tracking-ll-2}
	\end{algorithm}


==> code-ISB-LL2.tex <==


%\newcommand{\Iinfo}{\mbox{IInfo}}
%\newcommand{\Dinfo}{\mbox{DInfo}}
%\newcommand{\insertCode}[1]{{\color{green} #1}\normalcolor}
%\newcommand{\deleteCode}[1]{{\color{purple} #1}\normalcolor}


\begin{algorithm*}[tb]
	
	\nonl
	
	\begin{multicols*}{2}
	
	\SetKwBlock{Begin}{}{}	
		
	\removelatexerror
	\scriptsize

	\vspace{-6mm}
	%%%%%%%%%%%%%% Recoverable Linked List - Insert %%%%%%%%%%%%%%%%%%%%%%%%%
	
	\begin{procedure}[H]
		\caption{() \small boolean \insertlst\ (T $key$)}
		
		%Node *$pred$, *$curr$ \label{ISB-ll-Template2-insert-entry}\;
		%Update $predupdate, currupdate, result$ \;
		%Info *$result$, *$predInfo$, *$currInfo$ \;
		Node *\textit{newcurr} := \textbf{new} Node ($\init, \NULL, \NULL$) \; % \tcp*{copy for the successor of the new node} \label{ISB-ll-Template2-insert-create-newcurr}
		Node *\textit{newnd} := \textbf{new} Node (\textit{key}, \textit{newcurr}, $\NULL$) \label{ISB-ll-Template2-insert-create-newnd} \;
%		\yyy{Info *\textit{opInfo} := \textbf{new} \Info\ () \;}
		%($\insertlst, \NULL, \NULL, \NULL, \NULL, \bot$) \;
%		\flushcode{\pwb\ (all fields)} \;
		
		\recovercode{$RD_q$ := $\init$} \label{ISB-ll-Template2-insert-set-RDp} \;
		\flushcode{\pbarrier\ ($RD_q$)} \;
		\recovercode{$\text{CP}_q := 1$} \tcp*{check-point; $RD_q$ is initialized} \label{ISB-ll-Template2-insert-set-checkpoint}
		\flushcode{\pwb\ ($\text{CP}_q$)} \;
		\flushcode{\psync} \;
		
		
		\While{\True}{
			\Begin (\textbf{Gather Phase} \tcp*[f]{search for right location to insert})  {
				$\langle$ \textit{pred}, \textit{curr}, \textit{predInfo}, \textit{currInfo} $\rangle := \search(\textit{key})$  \label{ISB-ll-Template2-insert-call-search}
			}
			\Begin (\textbf{Helping Phase} \tcp*[f]{help other operations if necessary}) {
				\lIf {\textit{isTagged}(\textit{predInfo})} {\func{Help} ($predInfo$) \label{ISB-ll-Template2-insert-help-pred}}
				\lElseIf {\textit{isTagged}(\textit{currInfo})} {\func{Help} ($currInfo$) \label{ISB-ll-Template2-insert-help-curr}}
				\lIf {\textit{isTagged}(\textit{predInfo}) \OR IsTagged(currInfo)} { \Continue }
			}
			\uIf (\tcp*[f]{\textit{key} in list}) {\textit{curr} $\rightarrow$ \textit{key} = \textit{key}} {
				\recovercode{\textit{opInfo} $\rightarrow$ \textit{result} $:= \False$} \;
				\flushcode{\pbarrier\ (\textit{opInfo} $\rightarrow$ \textit{result})} \;
				\recovercode{$RD_q$ := \textit{opInfo}} \tcp*{persist response} \label{ISB-ll-Template2-insert-persist-false}
				\flushcode{\pwb\ ($RD_q$)} \;
				\flushcode{\psync} \;					
				\KwRet \False \label{ISB-ll-Template2-insert-return-false}
			}
			*\textit{opInfo} := \textbf{new} \Info\ (\insertlst, pred, curr, predInfo, currInfo, newnd, $\init$) \label{ISB-ll-Template2-delete-create-info} \;
%			\yyy{*\textit{opInfo} := $\langle$\insertlst, pred, curr, predInfo, currInfo, newnd, $\init \rangle$ \label{ISB-ll-Template2-delete-create-info} \;}
			\textit{newcurr} $\rightarrow$ \textit{key} $:=$ \textit{curr} $\rightarrow$ \textit{key} \label{ISB-ll-Template2-insert-update-newcurr-key} \;
			\textit{newcurr} $\rightarrow$ \textit{next} $:=$ \textit{curr} $\rightarrow$ \textit{next} \label{ISB-ll-Template2-insert-update-newcurr-next} \;
			\textit{newcurr} $\rightarrow$ \textit{info} $:=$ \textit{getTagged}(\textit{opInfo}) \;
			\textit{newnd} $\rightarrow$ \textit{info} := \textit{getTagged}(\textit{opInfo}) \;
			\flushcode{\pbarrier\ (\textit{newcurr}, \textit{newnd}, \textit{opInfo})} \;
			\recovercode{$RD_q$ := \textit{opInfo}} \tcp*{info for current attempt} \label{ISB-ll-Template2-delete-update-RD}
			\flushcode{\pwb\ ($RD_q$)} \;
			\flushcode{\psync} \;
			
			\func{Help}(\textit{opInfo}, {\color{orange}\True}) \;
			\uIf {\textit{opInfo} $\rightarrow$ \textit{result} $\neq \init$} {
				\KwRet \textit{opInfo} $\rightarrow$ \textit{result}
			}
%			\yyy{\textit{opInfo} := \textbf{new} \Info\ ()\;}
		}
	\end{procedure}
	
	\vfill\null
	\columnbreak
	
	%%%%%%%%%%%%%% Recoverable Linked List - Delete %%%%%%%%%%%%%%%%%%%%%%%%%
	
	\begin{procedure}[H]
		\caption{() boolean \delete\ (T $key$)}
		
		%Node *pred, *curr \;
		%Info *result, *predInfo, *currInfo \;
%		\yyy{Info *\textit{opInfo} := \textbf{new} \Info\ () \;}
		%($\delete, \NULL, \NULL, \NULL, \NULL, \init$) \label{ISB-ll-Template2-delete-create-info} \;
%		\flushcode{\pbarrier\ (all fields)} \;
		
		\recovercode{$RD_q$ := $\init$} \label{ISB-ll-Template2-delete-set-RD-init} \;
		\flushcode{\pbarrier\ ($RD_q$)} \;
		\recovercode{$\text{CP}_q := 1$} \tcp*{check-point; $RD_q$ is initialized} \label{ISB-ll-Template2-delete-set-checkpoint}
		\flushcode{\pwb\ ($\text{CP}_q$)} \;
		\flushcode{\psync} \;
		
		\While{\True}{
			\Begin (\textbf{Gather Phase} \tcp*[f]{search for node to delete})  {
				$\langle$\textit{pred}, \textit{curr}, \textit{predInfo}, \textit{currInfo}$\rangle :=$ \search(\textit{key}) \label{ISB-ll-Template2-delete-search}
			}
			\Begin (\textbf{Helping Phase} \tcp*[f]{help other operations if necessary}) {
				\lIf {\textit{isTagged}(\textit{predInfo})} {\func{Help}(\textit{predInfo}) \label{ISB-ll-Template2-delete-help-pred}}
				\lElseIf {\textit{isTagged}(\textit{currInfo}} {\func{Help}(\textit{currInfo}) \label{ISB-ll-Template2-delete-help-curr}}
				\lIf {\textit{isTagged}(\textit{predInfo}) \OR \textit{isTagged}(\textit{currInfo})} { \Continue }
				
			}
			\uIf (\tcp*[f]{\textit{key} not in the list}) {\textit{curr} $\rightarrow$ \textit{key} $\neq$ \textit{key} \label{ISB-ll-Template2-delete-if-in-list}} {
				\recovercode{\textit{opInfo} $\rightarrow$ \textit{result} $:=$ \False} \;
				\flushcode{\pbarrier\ (\textit{opInfo}$\rightarrow$ \textit{result})} \;
				\recovercode{$RD_q$ := \textit{opInfo}} \tcp*{persist response} \label{ISB-ll-Template2-delete-persist-false}
				\flushcode{\pwb\ ($RD_q$)} \;
				\flushcode{\psync} \;
				\KwRet \False \label{ISB-ll-Template2-delete-return-false}
			}
			*\textit{opInfo} := \textbf{new} \Info\ (\delete, \textit{pred}, \textit{curr}, \textit{predInfo}, \textit{currInfo}, \textit{curr} $\rightarrow$ \textit{next}, $\init$) \label{ISB-ll-Template2-delete-create-info} \;
%			\yyy{*\textit{opInfo} := $\langle$\delete, pred, curr, predInfo, currInfo, $curr \rightarrow next$, $\init \rangle$ \label{ISB-ll-Template2-delete-create-info} \;}
			\flushcode{\pbarrier\ (\textit{opInfo})} \;
			\recovercode{$RD_q$ := \textit{opInfo}} \tcp*{info for current attempt} \label{ISB-ll-Template2-delete-update-RD}
			\flushcode{\pwb\ ($RD_q$)} \;			
			\flushcode{\psync} \;
			\func{Help}(\textit{opInfo}, {\color{orange}\textit{TRUE}}) \;
			\uIf {\textit{opInfo} $\rightarrow$ \textit{result} $\neq \init$} {
				\KwRet \textit{opInfo} $\rightarrow$ \textit{result}
			}
%			\yyy{\textit{opInfo} := \textbf{new} \Info\ ()\;}
		}
	\end{procedure}


	\end{multicols*}

	\caption{Recoverable Linked List - \insertlst{} and \delete{}  (code for process $q$)}
%: \insertlst{}, \func{Op-Recover} \& \func{CompleteOp}}
	\label{alg:ISB-ll-Template2-insert-delete}
\end{algorithm*}

\begin{algorithm*}[tb]
	
	%\nonl
	
	\begin{multicols*}{2}
		
		\removelatexerror
		\scriptsize
		
		\SetKwBlock{Begin}{}{}		
		
		\begin{flushleft}
			
		type Node \{ \hspace*{13.25mm}  \\
		\hspace*{6mm} $\Key \cup \{\infty, -\infty\}$ $key$ \\
		\hspace*{6mm} Node *$next$ \\
		\hspace*{6mm} Info *$info$ \\
		\}
		
		
		type \Info\ \{ \\
		%\hspace*{6mm} \lefteris{\{\deletetag, \inserttag\} $type$} \\
		\hspace*{6mm} \{\delete, \insertlst, \find \} opType \\
		\hspace*{6mm} Node *$pred$, *$curr$; \\
		\hspace*{6mm} Info *$predInfo$, *$currInfo$ \\
		\hspace*{6mm} Node *$newptr$ \\ 	 %\hspace*{2cm} // used for Insert \\
		%\hspace*{6mm} Info *$currInfo$ \\
		\hspace*{6mm} \recovercode{boolean $result$} \\
		\}
		

		%\vspace*{-5mm}
		\com Initialization: \\
		\hspace*{6mm} Shared Node: *$head$ with key $-\infty$, *$tail$ with key $\infty$. \\
		\hspace*{6mm} $head \rightarrow next$ points to $tail$,  $tail \rightarrow next$ points to \NULL. \\
		\hspace*{6mm} Both $info$ fields are \NULL. \\
		
				\end{flushleft}
		
		
		%%%%%%%%%%%%%%%%%%%%%% Linked List - Search %%%%%%%%%%%%%%%%%%%%%%%%
		
		\begin{procedure}[H]
			\caption{() \small $\langle$ Node$^*$, Node$^*$, Info$^*$, Info$^*$ $\rangle$ \search\ (T $key$)}
			
			Node *$pred$, *$curr$ \;
			Info *$predInfo$, *$currInfo$ \;
			%	Update $predupdate$, $currupdate$ \;
			
			$curr := head$ \;
			$currInfo := head \rightarrow info$ \;
			%	$currupdate := curr.update$ \;
			\tcc{Search for first node with key $\geq$ $key$}
			\While{$curr \rightarrow key < key$}{
				$pred := curr$ \tcp*{remember predecessor}
				$predInfo := currInfo$ \tcp*{remember $info$ field of predecessor}
				$curr := curr \rightarrow next$ \tcp*{move forward in the list}
				$currInfo := curr\rightarrow info$ \tcp*{copy $info$ field}
			}
			\KwRet $\langle pred,curr, predInfo,currInfo \rangle$
		\end{procedure}
		
		%%%%%%%%%%%%%%%%%%%%%% Linked List - Find %%%%%%%%%%%%%%%%%%%%%%%%
		
		\begin{procedure}[H]
			\caption{() boolean \find\ (T $key$)}
			
			%Node *$nd$ \label{ISB-ll-Template2-find-start} \;
			%\tcc{Search for first node with key $\geq$ $key$}
			\While {\True} {
				\Begin (\textbf{Gather Phase}) {
					$\langle -, \textit{nd}, -, \textit{ndInfo} \rangle := \search\ (\textit{key})$ \;
				}
				\Begin (\textbf{Helping Phase}) {
					\uIf {IsTagged(\textit{ndinfo})} {
						\func{Help}(\textit{ndinfo}, {\color{orange} \False)} \;
						\Continue
					}
				}
				\yyy{\textit{result} $:=$ (\textit{nd} $\rightarrow$ \textit{key} $=$ \textit{key}) \;
				*\textit{opInfo} := \textbf{new} \Info\ (\find, \NULL, \NULL, \NULL, \NULL, \NULL, \textit{result}) \;}
				\flushcode{\pbarrier\ (\textit{opInfo})} \;
				\recovercode{$RD_q$ := \textit{opInfo}} \;
				\flushcode{\pwb\ ($RD_q$)} \;
				\flushcode{\psync} \;
				\yyy{\KwRet \textit{result}}
			}
		\end{procedure}
	
		
		%\vfill\null
		\columnbreak
		
		%%%%%%%%%%%%% Linked-List - Help-Op %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\begin{procedure}[H]
			\caption{() \mbox{ \small \func{Help} (\Info\ *\textit{opInfo}, {\color{orange} boolean \textit{invoker}})}}
			
			%Info *$result$ \;
			%Node *$other$ \;
			%\lIf {!IsTagged(\textit{opInfo})} {return \True}
			\Begin (\textbf{Tagging Phase} ) {
				{\color{orange} \uIf (\tcp*[f]{Try to tag \textit{pred}}) {\textit{invoker} $=$ \True } {
					{\color{black} \textit{result} $:=$ \CAS (\textit{opInfo} $\rightarrow$ \textit{pred} $\rightarrow$ \textit{info}, \textit{opInfo} $\rightarrow$ \textit{predInfo}, \textit{getTagged}(\textit{opInfo})) \tcp*{\textbf{tag} \CAS} \label{ISB-ll-Template2-HelpOp-pred-tag-CAS}}
					\flushcode{\pwb\ (\textit{opInfo} $\rightarrow$ \textit{pred} $\rightarrow$ \textit{info})} \;
					{\color{black}\uIf (\tcp*[f]{\textit{opInfo} $\rightarrow$ \textit{pred} is not tagged}) {\textit{result} $\neq$ \textit{opInfo} $\rightarrow$ \textit{predInfo} \AND \textit{result} $\neq$ \textit{getTagged}(\textit{opInfo})} {
						\KwRet
					}}			
				}}
				
				\tcc{Try to tag \textit{curr} for removal}
				\textit{result} $:=$ \CAS (\textit{opInfo} $\rightarrow$ \textit{curr} $\rightarrow$ \textit{info}, \textit{opInfo} $\rightarrow$ \textit{currInfo}, \textit{getTagged}(\textit{opInfo})) \tcp*{\textbf{tag} \CAS} \label{ISB-ll-Template2-HelpOp-curr-mark-CAS}
				\flushcode{\pwb\ (\textit{opInfo} $\rightarrow$ \textit{curr} $\rightarrow$ \textit{info})} \;
				\uIf (\tcp*[f]{\textit{opInfo} $\rightarrow$ \textit{curr} is not tagged}) {\textit{result} $\neq$ \textit{opInfo} $\rightarrow$ \textit{currInfo} \AND \textit{result} $\neq$ \textit{getTagged}(\textit{opInfo})} {
					\Begin (\textbf{Backtrack Phase}) {
						\CAS (\textit{opInfo} $\rightarrow$ \textit{pred} $\rightarrow$ \textit{info}, \textit{getTagged}(\textit{opInfo}), \textit{opInfo}) \;
						\flushcode{\pwb\ (\textit{opInfo} $\rightarrow$ \textit{pred} $\rightarrow$ \textit{info})} \;
						\flushcode{\psync\ ()} \;
						\KwRet \tcp*{operation attempt failed}
					}
				}
				\flushcode{\psync\ ()} \;
			}
			\Begin (\textbf{Update Phase} \tcp*[f]{update \textit{pred} $\rightarrow$ \textit{next}}) {
				\CAS(\textit{opInfo} $\rightarrow$ \textit{pred} $\rightarrow$ \textit{next},\textit{opInfo} $\rightarrow$ \textit{curr}, \textit{opInfo} $\rightarrow$ \textit{newptr}) \label{ISB-ll-Template2-CompleteTagged-CAS} \;
				\flushcode{\pwb\ (\textit{opInfo} $\rightarrow$ \textit{pred} $\rightarrow$ \textit{next})} \;
			}
			\tcc{complete operation}
			\recovercode{\textit{opInfo} $\rightarrow$ \textit{result} $:=$ \True} \tcp*{update response} \label{ISB-ll-Template2-CompleteTagged-set-result}
			\flushcode{\pwb\ (\textit{opInfo} $\rightarrow$ \textit{result})} \;
			\flushcode{\psync\ ()} \;
			
			\Begin (\textbf{Cleanup Phase}) {
				\CAS(\textit{opInfo} $\rightarrow$ \textit{pred} $\rightarrow$ \textit{info}, \textit{getTagged}(\textit{opInfo}), \textit{opInfo}) \label{ISB-ll-Template2-CompleteTagged-untag-CAS}\;
				\flushcode{\pwb\ (\textit{opInfo} $\rightarrow$ \textit{pred} $\rightarrow$ \textit{info})} \;
				\uIf {\textit{opInfo} $\rightarrow$ \textit{opType} = \insertlst} {
					\CAS(\textit{opInfo} $\rightarrow$ \textit{newptr} $\rightarrow$ \textit{info}, \textit{getTagged}(\textit{opInfo}), \textit{opInfo}) \;
					\flushcode{\pwb\ (\textit{opInfo} $\rightarrow$ \textit{newptr} $\rightarrow$ \textit{info})} \;
					\CAS(\textit{opInfo} $\rightarrow$ \textit{newptr} $\rightarrow$ \textit{next} $\rightarrow$ \textit{info}, \textit{getTagged}(\textit{opInfo}), \textit{opInfo}) \;
					\flushcode{\pwb\ (\textit{opInfo} $\rightarrow$ \textit{newptr} $\rightarrow$ \textit{next $\rightarrow$ \textit{info)}} \;
					}
				\flushcode{\psync ()} \;
			}}
			\KwRet \label{ISB-ll-Template2-CompleteOp-return-true}
					
		\end{procedure}
		
		
		%%%%%%%%%%%%% Linked List - Op-Recover %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\begin{procedure}[H]
			\color {blue} {
				\caption{() \small boolean \func{Op-Recover} (T $key$)}
				
				\Info\ *\textit{opInfo} := $RD_q$ \label{ISB-ll-Template2-OpRecover-read-RDp} \;
				
				\uIf {$CP_q = 0$ or \textit{opInfo} = $\init$} {
					Re-invoke \func{Op} \label{ISB-ll-Template2-OpRecover-first-reinvoke}
				}
%				\uIf {\textit{opInfo} $\rightarrow$ result = \False}
%				{\KwRet \False \tcp*[f]{false response is persisted} \label{ISB-ll-Template2-OpRecover-return-false}}

%				\yyy{\textit{test} $:=$ \textit{opInfo} $\rightarrow$ \textit{pred} $\rightarrow$ \textit{info} \label{ISB-ll-Template2-OpRecover-read-pred-update} \;
%				\uIf (\tcp*[f]{operation in progress;}){\textit{test} = \textit{getTagged}(\textit{opInfo}) } {
%					\func{CompleteOp}(\textit{opInfo}) \tcp*{complete it or untag}
%					\label{ISB-ll-Template2-OpRecover-call-CompleteOp}
%				}}

				\func{Help}(\textit{opinfo}, {\color{orange} \True)}

				\color {blue} {\uIf (\tcp*[f]{operation completed}) {\textit{opInfo} $\rightarrow$ \textit{result} $\neq \init$}
				{\KwRet \textit{opInfo} $\rightarrow$ \textit{result} \label{ISB-ll-Template2-OpRecover-return-true}}
				\lElse {
					Re-invoke \func{Op} \tcp*[f]{operation attempt failed} \label{ISB-ll-Template2-OpRecover-reinvoke}
				}}
			}
		\end{procedure}

	\end{multicols*}

	\caption{Recoverable Linked List - \func{Find}, \func{Op-Recover} and auxiliary functions (code for process $q$)}
	%\func{Search}, \func{Find}, \func{CompleteOp} and \func{Op-Recover}
	\label{alg:ISB-ll-Template2-recover} \label{alg:ISB-ll-Template2-search}
\end{algorithm*}

==> code-ISB-Queue-2col.tex <==

\begin{figure*}
	\removelatexerror
	
	\footnotesize
	\begin{flushleft}
		
		%type Update \{ \hspace*{14mm} \com stored in one CAS word \\
		%\hspace*{6mm} $\{\clean,\mk\}$ $state$ \\
		%\hspace*{6mm} Info *{\it info} \\
		%\}
		\begin{multicols*}{2}
		
		type Node \{ \hspace*{13.25mm}  \\
		\hspace*{6mm} $\Key\ key$ \\
		\hspace*{6mm} Node *$next$ \\
		\hspace*{6mm} Info *$info$ \\
		\} \\
		
		\columnbreak
		
		type \EnFlag\ \{ \hspace*{14.7mm} \com subtype of \Info \\
		\hspace*{6mm} Node *$tail$, *$new$ \\
		\hspace*{6mm} boolean $result$ \\
		\} \\
		%\columnbreak
		
		type \DeFlag\ \{ \hspace*{13.4mm} \com subtype of \Info \\
		\hspace*{6mm} Node *$head$ \\
		\hspace*{6mm} $\Key\ result$ \\
		\}
	\end{multicols*}

		\com Initialization: \\
		\hspace*{6mm} shared Nodes *$Head$ and *$Tail$, both points to a new allocated node\\
		\hspace*{6mm} with all fields initialize to \NULL.\\
	\end{flushleft}	
	\caption{Recoverable Queue: type definitions and initialization.}
	\label{ISB-Queue-types}
\end{figure*}



%%%%%%%%%%%%% RECOVER FUNCTIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm*}[tb]

	\nonl

	\begin{multicols*}{2}
	
	\removelatexerror
	\scriptsize

	%%%%%%%%%%%%% ENQUEUE-RECOVER FUNCTIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	\begin{procedure}[H]
		\caption{() boolean \func{Enqueue-Recover} ($\Key\ key$)}
		
		\EnFlag\ *$OpInfo := RD_p$ \;
		
		\uIf {$CP_p = 0$ or $OpInfo = \init$} {
			Re-invoke \enqueue \;
		}
		$test$ := $OpInfo \rightarrow tail \rightarrow info$ \;
		\uIf {$test = GetTagged(OpInfo)$} {
			\func{HelpEnqueue}$(OpInfo)$ \tcp*[f]{enqueue in progress; complete it}
		}
		\uIf (\tcp*[f]{enqueue completed successfully}) {$OpInfo \rightarrow result \neq \init$} {
			\KwRet $OpInfo \rightarrow result$
		}
		\lElse {Re-invoke \enqueue \tcp*[f]{enqueue attempt failed}}
	\end{procedure}
	
	%%%%%%%%%%%%% DELETE-RECOVER FUNCTIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	\begin{procedure}[H]
		\caption{() \Key\ \func{Dequeue-Recover} ()}
		
		\DeFlag\ *$OpInfo = RD_p$ \;
		
		\uIf {$CP_p = 0$ or $OpInfo = \init$} {
			Re-invoke \dequeue
		}
		\uIf (\tcp*[f]{observed an empty queue}) {$OpInfo \rightarrow result = \emptyst$} {\KwRet \emptyst}
		$test$ := $OpInfo \rightarrow head \rightarrow info$ \;
		\uIf {$test = GetTagged(OpInfo)$} {
			\func{HelpDequeue}$(OpInfo)$ \tcp*[f]{dequeue in progress; complete it}
		}
		\uIf (\tcp*[f]{dequeue completed successfully}) {$OpInfo \rightarrow result \neq \init$} {
			\KwRet $OpInfo \rightarrow result$
		}
		\lElse {Re-invoke \dequeue \tcp*[f]{dequeue attempt failed}}
	\end{procedure}
	
	\end{multicols*}
	
	\caption{Recoverable Queue: \func{Recover} functions}
	\label{ISB-Queue-recovery-functions}
\end{algorithm*}
	
\begin{algorithm*}[tb]
	\nonl

	\begin{multicols*}{2}
		
	\removelatexerror
	\scriptsize
	
	%%%%%%%%%%%%%% Recoverable Queue - Enqueue %%%%%%%%%%%%%%%%%%%%%%%%%

	\begin{procedure}[H]
		\caption{() boolean \enqueue\ ($\Key\ key$)}
		
		Node *$tail$ \label{insert-enqueue}\;
		Info *$tailInfo$, *$result$ \;
		Node *$newnd$ := \textbf{new} Node $\langle key, \NULL, \NULL \rangle$ \tcp*{new node to insert}
		
		$RD_p$ := $\init$ \;
		$CP_p := 1$ \tcp*{set a check-point indicating \Info\ structure was installed} \label{Queue-enqueue-set-checkpoint}
		
		\While{\True}{
			$tail := Tail$ \;
			$tailInfo := tail \rightarrow info$ \;
			
			\lIf (\tcp*[f]{Tail under changes; help the other operation}) {IsTagged($tailInfo$)} {\func{Help}($tailInfo$)}
			\uElse {
				*\textit{OpInfo} := \textbf{new} \EnFlag\ record, containing $\langle tail, newnd, \init \rangle$ \;
				$RD_p$ := \textit{OpInfo} \tcp*{update Info structure for current attempt}
				$result$ := \CAS\ ($tail \rightarrow info$, $tailInfo$, GetTagged(\textit{OpInfo}) \tcp*{\textbf{enflag} \CAS}
				\uIf (\tcp*[f]{the enflag \CAS\ was successful}) {$result = tailInfo$} {
					\func{HelpEnqueue}(\textit{OpInfo}) \tcp*{finish enqueue}
					\KwRet \True
				}
				\lElse (\tcp*[f]{the enflag \CAS\ failed; help the operation that caused failure}) {\func{Help}$(result)$}
			}
		}
	\end{procedure}

	\vfill\null
	\columnbreak

	%%%%%%%%%%%%%%%%%%%%%%%%%%%% HELP-ENQUEUE FUNCTION %%%%%%%%%%%%%%%%%%%%%

	\begin{procedure}[H]
		\caption{() boolean \func{HelpEnqueue} (\EnFlag\ *$OpInfo$)}
		
		Node *$tail := OpInfo \rightarrow tail$ \;
		Node *$newnd := OpInfo \rightarrow newnd$ \;
		
		$\CAS\ (tail \rightarrow next, \NULL, newnd)$ \tcp*{attach $newnd$ to the tail of the list}
		$\CAS (Tail, tail, newnd)$ \tcp*{swing Tail to the new node}
		$OpInfo \rightarrow result := \True$ \tcp*{announce the operation completed}
		\CAS ($tail \rightarrow info$, $OpInfo$, GetUntagged($OpInfo$)) \tcp*{\textbf{unflag} \CAS}
	\end{procedure}


	%%%%%%%%%%%%%% Recoverable Queue - Dequeue %%%%%%%%%%%%%%%%%%%%%%%%%

	\begin{procedure}[H]
		\caption{() $\Key$ \dequeue\ ()}
		
		Node *$head$ \label{dequeue-entry}\;
		Info *$headInfo$, *$result$ \;
		
		$RD_p$ := $\init$ \;
		$CP_p := 1$ \tcp*{set a check-point indicating \Info\ structure was installed} \label{Queue-dequeue-set-checkpoint}
		
		\While{\True}{
			$head := Head$ \;
			$headInfo := head \rightarrow info$ \;
			
			\lIf (\tcp*[f]{Head under changes; help the other operation}) {IsTagged($headInfo$)} {\func{Help}($headInfo$)}
			\uElseIf (\tcp*[f]{queue is empty}) {$headInfo = \NULL$} {
				$RD_p$ := pointer to a new \DeFlag\ record, with $result$ field \emptyst \tcp*{persist response}
				\KwRet \emptyst \;	
			}
			\uElse {
				$OpInfo$ := pointer to a new \DeFlag\ record, containing $\langle head, \init \rangle$ \;
				$RD_p$ := $OpInfo$ \tcp*{update Info structure for current attempt}
				$result$ := \CAS\ ($head \rightarrow info$, $headInfo$, GetTagged($OpInfo$)) \tcp*{\textbf{deflag} \CAS}
				\uIf (\tcp*[f]{the deflag \CAS\ was successful}) {$result = headInfo$} {
					\KwRet \func{HelpDequeue}$(OpInfo)$ \tcp*{finish dequeue}
				}
				\lElse (\tcp*[f]{the deflag \CAS\ failed; help the operation that caused failure}) {\func{Help}$(result)$}
			}
		}
	\end{procedure}
	
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%% HELP-DEQUEUE FUNCTION %%%%%%%%%%%%%%%%%%%%%
	
	\begin{procedure}[H]
		\caption{() \Key\ \func{HelpDequeue} (\DeFlag\ *$OpInfo$)}
		
		Node *$head := OpInfo \rightarrow head$ \;
		
		$H\CAS (Head, head, head \rightarrow next)$ \tcp*{swing Head to the next node}
		$OpInfo \rightarrow result := head \rightarrow next \rightarrow key$ \tcp*{persist response}
		\KwRet $OpInfo \rightarrow result$ \;
	\end{procedure}
	
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%% HELP FUNCTION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	\begin{procedure}[H]
		\caption{() \func{Help} (Info *$OpInfo$)}
		
		\nonl \com General-purpose helping routine \;
		%\Info\ *$op$ := $u.\info$ \;
		\lIf (\tcp*[f]{no help is needed}) {!IsTagged($OpInfo$)} {\KwRet}
		\lIf {$OpInfo$ of type \EnFlag} {\func{HelpEnqueue}$(OpInfo)$}
		\lElse {\func{HelpDequeue}$(OpInfo)$}
	\end{procedure}

	\end{multicols*}

\caption{Recoverable Queue: \enqueue\ and \dequeue}
\label{alg:ISB-Queue}
\end{algorithm*}




==> code-ISB-Queue.tex <==

\begin{figure*}
	\removelatexerror
	
	\footnotesize
	\begin{flushleft}
		
		%type Update \{ \hspace*{14mm} \com stored in one CAS word \\
		%\hspace*{6mm} $\{\clean,\mk\}$ $state$ \\
		%\hspace*{6mm} Info *{\it info} \\
		%\}
		\begin{multicols*}{2}
		
		type Node \{ \hspace*{13.25mm}  \\
		\hspace*{6mm} $\Key\ key$ \\
		\hspace*{6mm} Node *$next$ \\
		\hspace*{6mm} Info *$info$ \\
		\} \\
		
		\columnbreak
		
		type \EnFlag\ \{ \hspace*{14.7mm} \com subtype of \Info \\
		\hspace*{6mm} Node *$tail$, *$new$ \\
		\hspace*{6mm} boolean $result$ \\
		\} \\
		%\columnbreak
		
		type \DeFlag\ \{ \hspace*{13.4mm} \com subtype of \Info \\
		\hspace*{6mm} Node *$head$ \\
		\hspace*{6mm} $\Key\ result$ \\
		\}
	\end{multicols*}

		\com Initialization: \\
		\hspace*{6mm} shared Nodes *$Head$ and *$Tail$, both points to a new allocated node\\
		\hspace*{6mm} with all fields initialize to \NULL.\\
	\end{flushleft}	
	\caption{Recoverable Queue: type definitions and initialization.}
	\label{ISB-Queue-types}
\end{figure*}



%%%%%%%%%%%%% RECOVER FUNCTIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

	\begin{algorithm}
		\nonl
		\footnotesize
		\removelatexerror
	
		%%%%%%%%%%%%% ENQUEUE-RECOVER FUNCTIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%
		
		\begin{procedure}[H]
			\caption{() boolean \func{Enqueue-Recover} ($\Key\ key$)}
			
			\EnFlag\ *$OpInfo := RD_p$ \;
			
			\uIf {$CP_p = 0$ or $OpInfo = \init$} {
				Re-invoke \enqueue \;
			}
			$test$ := $OpInfo \rightarrow tail \rightarrow info$ \;
			\uIf {$test = GetTagged(OpInfo)$} {
				\func{HelpEnqueue}$(OpInfo)$ \tcp*[f]{enqueue in progress; complete it}
			}
			\uIf (\tcp*[f]{enqueue completed successfully}) {$OpInfo \rightarrow result \neq \init$} {
				\KwRet $OpInfo \rightarrow result$
			}
			\lElse {Re-invoke \enqueue \tcp*[f]{enqueue attempt failed}}
		\end{procedure}
		
		%%%%%%%%%%%%% DELETE-RECOVER FUNCTIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		
		\begin{procedure}[H]
			\caption{() \Key\ \func{Dequeue-Recover} ()}
			
			\DeFlag\ *$OpInfo = RD_p$ \;
			
			\uIf {$CP_p = 0$ or $OpInfo = \init$} {
				Re-invoke \dequeue
			}
			\uIf (\tcp*[f]{observed an empty queue}) {$OpInfo \rightarrow result = \emptyst$} {\KwRet \emptyst}
			$test$ := $OpInfo \rightarrow head \rightarrow info$ \;
			\uIf {$test = GetTagged(OpInfo)$} {
				\func{HelpDequeue}$(OpInfo)$ \tcp*[f]{dequeue in progress; complete it}
			}
			\uIf (\tcp*[f]{dequeue completed successfully}) {$OpInfo \rightarrow result \neq \init$} {
				\KwRet $OpInfo \rightarrow result$
			}
			\lElse {Re-invoke \dequeue \tcp*[f]{dequeue attempt failed}}
		\end{procedure}
		
		\caption{Recoverable Queue: \func{Recover} functions}
		\label{ISB-Queue-recovery-functions}
	\end{algorithm}
	
\begin{algorithm}[tb]
	\nonl
	\removelatexerror

	\footnotesize
	
%%%%%%%%%%%%%% Recoverable Queue - Enqueue %%%%%%%%%%%%%%%%%%%%%%%%%

	\begin{procedure}[H]
		\caption{() boolean \enqueue\ ($\Key\ key$)}
		
		Node *$tail$ \label{insert-enqueue}\;
		Info *$tailInfo$, *$result$ \;
		Node *$newnd$ := \textbf{new} Node $\langle key, \NULL, \NULL \rangle$ \tcp*{new node to insert}
		
		$RD_p$ := $\init$ \;
		$CP_p := 1$ \tcp*{set a check-point indicating \Info\ structure was installed} \label{Queue-enqueue-set-checkpoint}
		
		\While{\True}{
			$tail := Tail$ \;
			$tailInfo := tail \rightarrow info$ \;
			
			\lIf (\tcp*[f]{Tail under changes; help the other operation}) {IsTagged($tailInfo$)} {\func{Help}($tailInfo$)}
			\uElse {
				*\textit{OpInfo} := \textbf{new} \EnFlag\ record, containing $\langle tail, newnd, \init \rangle$ \;
				$RD_p$ := \textit{OpInfo} \tcp*{update Info structure for current attempt}
				$result$ := \CAS\ ($tail \rightarrow info$, $tailInfo$, GetTagged(\textit{OpInfo}) \tcp*{\textbf{enflag} \CAS}
				\uIf (\tcp*[f]{the enflag \CAS\ was successful}) {$result = tailInfo$} {
					\func{HelpEnqueue}(\textit{OpInfo}) \tcp*{finish enqueue}
					\KwRet \True
				}
				\lElse (\tcp*[f]{the enflag \CAS\ failed; help the operation that caused failure}) {\func{Help}$(result)$}
			}
		}
	\end{procedure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%% HELP-ENQUEUE FUNCTION %%%%%%%%%%%%%%%%%%%%%

	\begin{procedure}[H]
		\caption{() boolean \func{HelpEnqueue} (\EnFlag\ *$OpInfo$)}
		
		Node *$tail := OpInfo \rightarrow tail$ \;
		Node *$newnd := OpInfo \rightarrow newnd$ \;
		
		$\CAS\ (tail \rightarrow next, \NULL, newnd)$ \tcp*{attach $newnd$ to the tail of the list}
		$\CAS (Tail, tail, newnd)$ \tcp*{swing Tail to the new node}
		$OpInfo \rightarrow result := \True$ \tcp*{announce the operation completed}
		\CAS ($tail \rightarrow info$, $OpInfo$, GetUntagged($OpInfo$)) \tcp*{\textbf{unflag} \CAS}
	\end{procedure}


%%%%%%%%%%%%%% Recoverable Queue - Dequeue %%%%%%%%%%%%%%%%%%%%%%%%%

\begin{procedure}[H]
	\caption{() $\Key$ \dequeue\ ()}
	
	Node *$head$ \label{dequeue-entry}\;
	Info *$headInfo$, *$result$ \;
	
	$RD_p$ := $\init$ \;
	$CP_p := 1$ \tcp*{set a check-point indicating \Info\ structure was installed} \label{Queue-dequeue-set-checkpoint}
	
	\While{\True}{
		$head := Head$ \;
		$headInfo := head \rightarrow info$ \;
		
		\lIf (\tcp*[f]{Head under changes; help the other operation}) {IsTagged($headInfo$)} {\func{Help}($headInfo$)}
		\uElseIf (\tcp*[f]{queue is empty}) {$headInfo = \NULL$} {
			$RD_p$ := pointer to a new \DeFlag\ record, with $result$ field \emptyst \tcp*{persist response}
			\KwRet \emptyst \;	
		}
		\uElse {
			$OpInfo$ := pointer to a new \DeFlag\ record, containing $\langle head, \init \rangle$ \;
			$RD_p$ := $OpInfo$ \tcp*{update Info structure for current attempt}
			$result$ := \CAS\ ($head \rightarrow info$, $headInfo$, GetTagged($OpInfo$)) \tcp*{\textbf{deflag} \CAS}
			\uIf (\tcp*[f]{the deflag \CAS\ was successful}) {$result = headInfo$} {
				\KwRet \func{HelpDequeue}$(OpInfo)$ \tcp*{finish dequeue}
			}
			\lElse (\tcp*[f]{the deflag \CAS\ failed; help the operation that caused failure}) {\func{Help}$(result)$}
		}
	}
\end{procedure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%% HELP-DEQUEUE FUNCTION %%%%%%%%%%%%%%%%%%%%%

\begin{procedure}[H]
	\caption{() \Key\ \func{HelpDequeue} (\DeFlag\ *$OpInfo$)}
	
	Node *$head := OpInfo \rightarrow head$ \;
	
	$H\CAS (Head, head, head \rightarrow next)$ \tcp*{swing Head to the next node}
	$OpInfo \rightarrow result := head \rightarrow next \rightarrow key$ \tcp*{persist response}
	\KwRet $OpInfo \rightarrow result$ \;
\end{procedure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%% HELP FUNCTION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{procedure}[H]
	\caption{() \func{Help} (Info *$OpInfo$)}
	
	\nonl \com General-purpose helping routine \;
	%\Info\ *$op$ := $u.\info$ \;
	\lIf (\tcp*[f]{no help is needed}) {!IsTagged($OpInfo$)} {\KwRet}
	\lIf {$OpInfo$ of type \EnFlag} {\func{HelpEnqueue}$(OpInfo)$}
	\lElse {\func{HelpDequeue}$(OpInfo)$}
\end{procedure}

\caption{Recoverable Queue: \enqueue\ and \dequeue}
\label{alg:ISB-Queue}
\end{algorithm}




==> code-ISB-linked-list-2col.tex <==


\newcommand{\Iinfo}{\mbox{IInfo}}
\newcommand{\Dinfo}{\mbox{DInfo}}
\newcommand{\insertCode}[1]{{\color{green} #1}\normalcolor}
\newcommand{\deleteCode}[1]{{\color{purple} #1}\normalcolor}

\begin{algorithm}[tb]
	
	\nonl
	
	\begin{multicols*}{2}
		
	\removelatexerror
	\scriptsize


	\vspace{-6mm}
	%%%%%%%%%%%%%% Recoverable Linked List - Insert %%%%%%%%%%%%%%%%%%%%%%%%%
	
	\begin{procedure}[H]
		\caption{() \small boolean \insertlst\ (T $key$)}
		
		Node *$pred$, *$curr$ \label{ISB-ll-insert-entry}\;
		%Update $predupdate, currupdate, result$ \;
		Info *$result$, *$predInfo$, *$currInfo$ \;
		Node *$newcurr$ := \textbf{new} Node ($\init, \NULL, \NULL$) \; % \tcp*{copy for the successor of the new node} \label{ISB-ll-insert-create-newcurr}
		Node *$newnd$ := \textbf{new} Node ($key, newcurr, \NULL$) \label{ISB-ll-insert-create-newnd} \;
		Info *\textit{OpInfo} := \textbf{new} \Info\ ($\insertlst, \NULL, \NULL, \NULL, \NULL, \bot$) \;
		
		\recovercode{$RD_q$ := $\init$} \label{ISB-ll-insert-set-RDp} \;
		\recovercode{$\text{CP}_q := 1$} \tcp*{check-point; $RD_q$ is initialized} \label{ISB-ll-insert-set-checkpoint}
		
		\While{\True}{
			$\langle pred, curr, predInfo,currInfo \rangle := \search(key)$ \tcp*{search for right location to insert} \label{ISB-ll-insert-call-search}
			\uIf (\tcp*[f]{$key$ in list}) {$curr \rightarrow key = key$} {
				\recovercode{$\textit{OpInfo} \rightarrow result$ := $\False$} \;
				\recovercode{$RD_q$ := \textit{OpInfo}} \tcp*{persist response} \label{ISB-ll-insert-persist-false}
				\KwRet \False \label{ISB-ll-insert-return-false}
			}
			\tcc{help other operations if neccessary:}
			\uIf {IsTagged(predInfo)} {\func{CompleteOp} ($predInfo$) \label{ISB-ll-insert-help-pred}}
			\uElseIf {IsTagged(currInfo)} {\func{CompleteOp} ($currInfo$) \label{ISB-ll-insert-help-curr}}
			\uElse {
				$newcurr\rightarrow key := curr \rightarrow key$ %  \tcp*{update copy of $curr$}
                                \label{ISB-ll-insert-update-newcurr-key} \;
				$newcurr\rightarrow next := curr\rightarrow next$ \label{ISB-ll-insert-update-newcurr-next} \;
				*\textit{OpInfo} := \textbf{new} \Info\  ($\insertlst, pred, curr, newnd, currInfo, \bot$) \label{ISB-ll-insert-create-info}\;
				\recovercode{$RD_q$ := \textit{OpInfo}} \tcp*{Info for current attempt} \label{ISB-ll-insert-update-RDp}
				$result$ := \CAS ($pred\rightarrow info$, $predInfo$, GetTagged(\textit{OpInfo})) \tcp*{\textbf{tag} \CAS} \label{ISB-ll-insert-tag-cas}
				\uIf (\tcp*[f]{successful tag}) {$result = predInfo$} {
					\tcc{either finish insertion or untag}
					\lIf { \func{CompleteOp}(getTagged(\textit{OpInfo}))}	{\KwRet \True \label{ISB-ll-insert-call-CompleteOp}} }
				\lElse (\tcp*[f]{tag \CAS\ failed; help the operation that caused failure}) {\func{CompleteOp}(result) \label{ISB-ll-insert-help-after-CAS}}
			}
		}
	\end{procedure}
	
	\vfill\null
	\columnbreak
	
	%%%%%%%%%%%%%% Recoverable Linked List - Delete %%%%%%%%%%%%%%%%%%%%%%%%%
	
	\begin{procedure}[H]
		\caption{() boolean \delete\ (T $key$)}
		
		Node *pred, *curr \;
		Info *result, *predInfo, *currInfo \;
		Info *\textit{OpInfo} := \textbf{new} \Info\ ($\delete, \NULL, \NULL, \NULL, \NULL, \init$) \label{ISB-ll-delete-create-info} \;
		
		\recovercode{$RD_q$ := $\init$} \label{ISB-ll-delete-set-RD-init} \;
		\recovercode{$\text{CP}_q := 1$} \tcp*{check-point; $RD_q$ is initialized} \label{ISB-ll-delete-set-checkpoint}
		
		\While{\True}{
			$\langle$ pred, curr, predInfo, currInfo $\rangle$ := \search(key) \tcp*{search for node to delete} \label{ISB-ll-delete-search}
			\uIf (\tcp*[f]{$key$ not in the list}) {curr$\rightarrow$key $\neq$ key \label{ISB-ll-delete-if-in-list}} {
				\recovercode{\textit{OpInfo}$\rightarrow$result := \False} \;
				\recovercode{$RD_q$ := \textit{OpInfo}} \tcp*{persist response} \label{ISB-ll-delete-persist-false}
				\KwRet \False \label{ISB-ll-delete-return-false}
			}
			\tcc{help other operations if neccessary}
			\uIf {IsTagged(predInfo)} {\func{CompleteOp}(predInfo) \label{ISB-ll-delete-help-pred}}
			\uElseIf {IsTagged(currInfo} {\func{CompleteOp}(currInfo) \label{ISB-ll-delete-help-curr}}
			\uElse {
				*\textit{OpInfo} := \textbf{new} \Info\ (\delete, pred, curr, \NULL, currInfo, $\init$) \label{ISB-ll-delete-create-info} \;
				\recovercode{$RD_q$ := \textit{OpInfo}} \tcp*{info for current attempt} \label{ISB-ll-delete-update-RD}
				result := \CAS (pred$\rightarrow$Info, predInfo, getTagged(\textit{OpInfo})) \tcp*{\textbf{tag} \CAS} \label{ISB-ll-delete-tag-CAS}
				\uIf (\tcp*[f]{successful tag}) {result = predInfo} {
					\tcc{either finish deletion or untag}
					\uIf {\func{CompleteOp}(getTagged(\textit{OpInfo}))}	{\KwRet \True \label{ISB-ll-delete-CompleteDelete}}
				}
				\lElse {\func{CompleteOp}(result) \tcp*[f]{tag \CAS\ failed; help the operation that caused failure} \label{ISB-ll-delete-help-after-CAS}}
			}
		}
	\end{procedure}


	\end{multicols*}

	\caption{Recoverable Linked List - \insertlst{} and \delete{}  (code for process $q$)}
%: \insertlst{}, \func{Op-Recover} \& \func{CompleteOp}}
	\label{alg:ISB-ll-insert-delete}
\end{algorithm}





\begin{algorithm}[tb]
	
	%\nonl
	
	\begin{multicols*}{2}
		
		\removelatexerror
		\scriptsize
		
		\begin{flushleft}
			
		type Node \{ \hspace*{13.25mm}  \\
		\hspace*{6mm} $\Key \cup \{\infty, -\infty\}$ $key$ \\
		\hspace*{6mm} Node *$next$ \\
		\hspace*{6mm} Info *$info$ \\
		\}
		
		
		type \Info\ \{ \\
		%\hspace*{6mm} \lefteris{\{\deletetag, \inserttag\} $type$} \\
		\hspace*{6mm} \{\delete, \insertlst\} opType \\
		\hspace*{6mm} Node *$pred$, *$curr$; \\
		\hspace*{6mm} Node *$new$ 	 \hspace*{2cm} // used for Insert \\
		\hspace*{6mm} Info *$currInfo$ \\
		\hspace*{6mm} \recovercode{boolean $result$} \\
		\}
		

		%\vspace*{-5mm}
		\com Initialization: \\
		\hspace*{6mm} Shared Node: *$head$ with key $-\infty$, *$tail$ with key $\infty$. \\
		\hspace*{6mm} $head \rightarrow next$ points to $tail$,  $tail \rightarrow next$ points to \NULL. \\
		\hspace*{6mm} Both $info$ fields are \NULL. \\
		
				\end{flushleft}
		
		
		%%%%%%%%%%%%%%%%%%%%%% Linked List - Search %%%%%%%%%%%%%%%%%%%%%%%%
		
		\begin{procedure}[H]
			\caption{() \small $\langle$ Node$^*$, Node$^*$, Info$^*$, Info$^*$ $\rangle$ \search\ (T $key$)}
			
			Node *$pred$, *$curr$ \;
			Info *$predInfo$, *$currInfo$ \;
			%	Update $predupdate$, $currupdate$ \;
			
			$curr := head$ \;
			$currInfo := head \rightarrow info$ \;
			%	$currupdate := curr.update$ \;
			\tcc{Search for first node with key $\geq$ $key$}
			\While{$curr \rightarrow key < key$}{
				$pred := curr$ \tcp*{remember predecessor}
				$predInfo := currInfo$ \tcp*{remember $info$ field of predecessor}
				$curr := curr \rightarrow next$ \tcp*{move forward in the list}
				$currInfo := curr\rightarrow info$ \tcp*{copy $info$ field}
			}
			\KwRet $\langle pred,curr, predInfo,currInfo \rangle$
		\end{procedure}
		
		%%%%%%%%%%%%%%%%%%%%%% Linked List - Find %%%%%%%%%%%%%%%%%%%%%%%%
		
		\begin{procedure}[H]
			\caption{() boolean \find\ (T $key$)}
			
			Node *$nd$ \label{ISB-ll-find-start} \;
			%\tcc{Search for first node with key $\geq$ $key$}
			$\langle -, nd, -, - \rangle := \search\ (key)$ \;
			\KwRet ($nd \rightarrow key = key$) \label{ISB-ll-find-end}
		\end{procedure}
	
		
		\vfill\null
		\columnbreak
		
		%%%%%%%%%%%%% Linked-List - Complete-Op %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\begin{procedure}[H]
			\caption{() \mbox{ \small boolean \func{CompleteOp} (\Info\ *\textit{OpInfo})}}
			
			Info *$result$ \;
			Node *$other$ \;
			
			
			\lIf {!IsTagged(\textit{OpInfo})} {return \True}
			\textit{utOpInfo} = GetUntagged(\textit{OpInfo}) \;
			
			\tcc{Set $other$ to the new node $pred$ needs to point to, according to the operation type}
			\uIf {\textit{utOpInfo}$\rightarrow$opType = \insertlst} {other := \textit{OpInfo}$\rightarrow$ new}
			\lElse {other := \textit{utOpInfo}$\rightarrow$curr$\rightarrow$next}
			
			\tcc{Try to tag $curr$ for removal}
			
			result := \CAS (\textit{utOpInfo}$\rightarrow$curr$\rightarrow$info, $\qquad$ \textit{utOpInfo}$\rightarrow$currInfo, \textit{OpInfo}) \tcp*{\textbf{tag} \CAS} \label{ISB-ll-CompleteOp-mark-CAS}
			\uIf (\tcp*[f]{\textit{OpInfo}$\rightarrow$curr is tagged}) {result = \textit{utOpInfo}$\rightarrow$currInfo or result = \textit{OpInfo}} {
				\tcc{update pred$\rightarrow$next; complete operation}
				\CAS(\textit{utOpInfo}$\rightarrow$pred$\rightarrow$next,\textit{utOpInfo}$\rightarrow$curr,other) \label{ISB-ll-CompleteTagged-CAS} \;
				\vspace*{-7pt}
				\recovercode{\textit{OpInfo}$\rightarrow$result := \True} \tcp*{update response} \label{ISB-ll-CompleteTagged-set-result}
				\CAS(\textit{utOpInfo}$\rightarrow$pred$\rightarrow$info, \textit{OpInfo}, \textit{utOpInfo}) \label{ISB-ll-CompleteTagged-untag-CAS}\;
				\KwRet \True \label{ISB-ll-CompleteOp-return-true}
			}
			\uElse (\tcp*[f]{tag \CAS\ failed; untag}) {
				%\uIf {flag} {\func{CompleteOp}(result, \False) \tcp*{help operation that caused failure} \label{ISB-ll-CompleteOp-help-after-CAS}}
				\CAS (\textit{utOpInfo}$\rightarrow$pred$\rightarrow$info, \textit{OpInfo}, \textit{utOpInfo}) \label{ISB-ll-CompleteOp-backtrack-CAS}
				\KwRet \False \tcp*{operation attempt failed} \label{ISB-ll-CompleteOp-return-false}
			}
		\end{procedure}
		
		
		%%%%%%%%%%%%% Linked List - Op-Recover %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\begin{procedure}[H]
			\color {blue} {
				\caption{() \small boolean \func{Op-Recover} (T $key$)}
				
				\Info\ *$\textit{OpInfo} := RD_q$ \label{ISB-ll-OpRecover-read-RDp} \;
				
				\uIf {$CP_q = 0$ or $\textit{OpInfo} = \init$} {
					Re-invoke \func{Op} \label{ISB-ll-OpRecover-first-reinvoke}
				}
				\uIf {$\textit{OpInfo} \rightarrow result = \False$}
				{\KwRet \False \tcp*[f]{false response is persisted} \label{ISB-ll-OpRecover-return-false}}
				$test := \textit{OpInfo} \rightarrow pred \rightarrow info$ \label{ISB-ll-OpRecover-read-pred-update} \;
				\uIf {$test = GetTagged(OpInfo)$} {
					\tcp*{operation in progress; complete it or untag}
					\func{CompleteOp}$(GetTagged(OpInfo))$
					\label{ISB-ll-OpRecover-call-CompleteOp}
				}
				\uIf (\tcp*[f]{operation completed}) {$\textit{OpInfo} \rightarrow result \neq \init$}
				{\KwRet $\textit{OpInfo} \rightarrow result$ \label{ISB-ll-OpRecover-return-true}}
				\lElse {
					Re-invoke \func{Op} \tcp*[f]{operation attempt failed} \label{ISB-ll-OpRecover-reinvoke}
				}
			}
		\end{procedure}

	\end{multicols*}

	\caption{Recoverable Linked List - \func{Find}, \func{Op-Recover} and auxiliary functions (code for process $q$)}
	%\func{Search}, \func{Find}, \func{CompleteOp} and \func{Op-Recover}
	\label{alg:ISB-ll-recover} \label{alg:ISB-ll-search}
\end{algorithm}


==> code-ISB-linked-list.tex <==


\newcommand{\Iinfo}{\mbox{IInfo}}
\newcommand{\Dinfo}{\mbox{DInfo}}
\newcommand{\insertCode}[1]{{\color{green} #1}\normalcolor}
\newcommand{\deleteCode}[1]{{\color{purple} #1}\normalcolor}

\begin{algorithm}

	\removelatexerror
	\scriptsize
	\begin{flushleft}
	\end{flushleft}	


\remove{
%%%%%%%%%%%%%% Recoverable Linked List - OP %%%%%%%%%%%%%%%%%%%%%%%%%

	\begin{procedure}[H]
		\caption{() boolean \func{Op} (T $key$)}
		
		Node *$pred$, *$curr$ \label{ISB-ll-insert-entry} \;
		%Update $predupdate, currupdate, result$ \;
		Info *$result$, *$predInfo$, *$currInfo$ \;
		Info *\textit{OpInfo} := \textbf{new} \Info ($\NULL, \NULL, \NULL, \bot, \bot$) \;
		\insertCode{
		\tcc{For \insertlst: allocate two new nodes}
		Node *$newcurr$ := \textbf{new} Node($\init, \NULL, \NULL$) % \tcp*{copy for the successor of the new node}
                        \label{ISB-ll-insert-create-newcurr}
                Node *$newnd$ := \textbf{new} Node ($key, newcurr, \NULL$) \label{ISB-ll-insert-create-newnd}
                }
		
		$RD_q$ := $\init$ \label{ISB-ll-insert-set-RDp} \;
		$\text{CP}_q := 1$ \tcp*{check-point; indicating $RD_q$ is initialized} \label{ISB-ll-insert-set-checkpoint}
		
		\While{\True}{
			$\langle pred, curr, predInfo,currInfo \rangle := \search(key)$ \tcp*{search for right location to insert or delete} \label{ISB-ll-insert-call-search}
			%(\tcp*[f]{$key$ already in the list})
			\uIf {\insertCode{\insertlst: $curr \rightarrow key = key$ \tcp*{$key$ already in the list}}
				\deleteCode{\delete: $curr \rightarrow key \neq key$ \tcp*{$key$ not in the list}}} {
				$\textit{OpInfo} \rightarrow result$ := $\False$ \;
				$RD_q$ := \textit{OpInfo} \tcp*{persist response} \label{ISB-ll-insert-persist-false}
				\KwRet \False \label{ISB-ll-insert-return-false}
			}
			\tcc{help other operations if neccessary:}
			\lIf {IsTagged(predInfo)} {\func{CompleteOp} ($predInfo$, \False) \label{ISB-ll-insert-help-pred}}
			\lElseIf {IsTagged(currInfo)} {\func{CompleteOp} ($currInfo$, \False) \label{ISB-ll-insert-help-curr}}
			\uElse {
				\insertCode{
					\tcp{For \insertlst: update the copy of $curr$}
				$newcurr\rightarrow key := curr \rightarrow key$ \label{ISB-ll-insert-update-newcurr-key} \;
				$newcurr\rightarrow next := curr\rightarrow next$
				 \label{ISB-ll-insert-update-newcurr-next} \;
				}
				*\textit{OpInfo} := pointer to a new allocated Info structure, with $opType = \func{Op}$, $pred,curr,currInfo$ as the corresponding fields, and $result = \bot$. For \insertlst\ $new = newnd$, and for \delete\ $new = \NULL$. \label{ISB-ll-insert-create-info} \;
				%$\langle pred, curr, newnd, currInfo, \bot \rangle$ \label{ISB-ll-insert-create-info}\;
				$RD_q$ := \textit{OpInfo} \tcp*{update Info structure for current attempt} \label{ISB-ll-insert-update-RDp}
				$result$ := \CAS ($pred\rightarrow info$, $predInfo$, GetTagged(\textit{OpInfo})) \tcp*{\textbf{tag} \CAS} \label{ISB-ll-insert-tag-cas}
				\uIf (\tcp*[f]{successful tag \CAS}) {$result = predInfo$} {
					\lIf (\tcp*[f]{either finish insertion or untag}) {\func{CompleteOp}(getTagged(\textit{OpInfo}))}	{\KwRet \True \label{ISB-ll-insert-call-CompleteOp}} }
				%\lElse (\tcp*[f]{the tag \CAS\ failed; help the operation that caused failure}) {\func{CompleteOp}(result, \False) \label{ISB-ll-insert-help-after-CAS}}
			}
		}
	\end{procedure}
}


	%%%%%%%%%%%%%% Recoverable Linked List - Insert %%%%%%%%%%%%%%%%%%%%%%%%%
	
	\begin{procedure}[H]
		\caption{() boolean \insertlst\ (T $key$)}
		
		Node *$pred$, *$curr$ \label{ISB-ll-insert-entry}\;
		%Update $predupdate, currupdate, result$ \;
		Info *$result$, *$predInfo$, *$currInfo$ \;
		Node *$newcurr$ := \textbf{new} Node($\init, \NULL, \NULL$) % \tcp*{copy for the successor of the new node} \label{ISB-ll-insert-create-newcurr}
		Node *$newnd$ := \textbf{new} Node ($key, newcurr, \NULL$) \tcp*{new node} \label{ISB-ll-insert-create-newnd}
		Info *\textit{OpInfo} := \textbf{new} \Info\ ($\NULL, \NULL, \NULL, \NULL, \bot$) \;
		
		\recovercode{$RD_q$ := $\init$} \label{ISB-ll-insert-set-RDp} \;
		\recovercode{$\text{CP}_q := 1$} \tcp*{check-point; indicating $RD_q$ is initialized} \label{ISB-ll-insert-set-checkpoint}
		
		\While{\True}{
			$\langle pred, curr, predInfo,currInfo \rangle := \search(key)$ \tcp*{search for right location to insert} \label{ISB-ll-insert-call-search}
			\uIf (\tcp*[f]{$key$ in list}) {$curr \rightarrow key = key$} {
				\recovercode{$\textit{OpInfo} \rightarrow result$ := $\False$} \;
				\recovercode{$RD_q$ := \textit{OpInfo}} \tcp*{persist response} \label{ISB-ll-insert-persist-false}
				\KwRet \False \label{ISB-ll-insert-return-false}
			}
			\tcc{help other operations if neccessary:}
			\lIf {IsTagged(predInfo)} {\func{CompleteOp} ($predInfo$) \label{ISB-ll-insert-help-pred}}
			\lElseIf {IsTagged(currInfo)} {\func{CompleteOp} ($currInfo$) \label{ISB-ll-insert-help-curr}}
			\uElse {
				$newcurr\rightarrow key := curr \rightarrow key$ % \tcp*{update copy of $curr$}
                                \label{ISB-ll-insert-update-newcurr-key}
				$newcurr\rightarrow next := curr\rightarrow next$ \label{ISB-ll-insert-update-newcurr-next} \;
				*\textit{OpInfo} := \textbf{new} \Info\  ($pred, curr, newnd, currInfo, \bot$) \label{ISB-ll-insert-create-info}\;
				\recovercode{$RD_q$ := \textit{OpInfo}} \tcp*{update Info for current attempt} \label{ISB-ll-insert-update-RDp}
				$result$ := \CAS ($pred\rightarrow info$, $predInfo$, GetTagged(\textit{OpInfo})) \tcp*{\textbf{tag} \CAS} \label{ISB-ll-insert-tag-cas}
				\uIf (\tcp*[f]{successful tag \CAS}) {$result = predInfo$} {
					\lIf (\tcp*[f]{either finish insertion or untag}) {\func{CompleteOp}(getTagged(\textit{OpInfo}))}	{\KwRet \True \label{ISB-ll-insert-call-CompleteOp}} }
				\lElse (\tcp*[f]{tag \CAS\ failed; help the operation that caused failure}) {\func{CompleteOp}(result) \label{ISB-ll-insert-help-after-CAS}}
			}
		}
	\end{procedure}

%\caption{Recoverable Linked List: \insertlst } \label{alg:ISB-ll-insert-delete}
%\end{algorithm}
%
%
%\begin{algorithm}[t]
%	
%	\removelatexerror
%	\scriptsize
%	\begin{flushleft}
%	\end{flushleft}	
%	
%
	\begin{procedure}[H]
		\caption{() boolean \func{CompleteOp} (\Info\ *\textit{OpInfo})}
		
		Info *result, Node *other \;
		

		\uIf {!IsTagged(\textit{OpInfo})} {return \True}
		\textit{utOpInfo} = GetUntagged(\textit{OpInfo}) \;

		\tcc{Set $other$ to the new node $pred$ needs to points to, according to the operation type}
		\lIf {\textit{utOpInfo}$\rightarrow$opType = \insertlst} {other := \textit{OpInfo}$\rightarrow$ new}
		\lElse {other := \textit{utOpInfo}$\rightarrow$curr$\rightarrow$next}

		\tcc{Try to tag $curr$ for removal}
		
		result := \CAS (\textit{utOpInfo}$\rightarrow$curr$\rightarrow$info, \textit{utOpInfo}$\rightarrow$currInfo, \textit{OpInfo}) \tcp*{\textbf{tag} \CAS} \label{ISB-ll-CompleteOp-mark-CAS}
		\uIf (\tcp*[f]{\textit{OpInfo}$\rightarrow$curr is tagged}) {result = \textit{utOpInfo}$\rightarrow$currInfo or result = \textit{OpInfo}} {
			\CAS (\textit{utOpInfo}$\rightarrow$pred$\rightarrow$next, \textit{utOpInfo}$\rightarrow$curr, other) \tcp*{swing $pred.next$ to $other$} \label{ISB-ll-CompleteTagged-CAS}
			\recovercode{\textit{OpInfo}$\rightarrow$result := \True} \tcp*{operation completed} \label{ISB-ll-CompleteTagged-set-result}
			\CAS(\textit{utOpInfo}$\rightarrow$pred$\rightarrow$info, \textit{OpInfo}, \textit{utOpInfo}) \tcp*{\textbf{untag} \CAS} \label{ISB-ll-CompleteTagged-untag-CAS}
			\KwRet \True \label{ISB-ll-CompleteOp-return-true}
		}
		\uElse (\tcp*[f]{tag \CAS\ failed}) {
			%\uIf {flag} {\func{CompleteOp}(result, \False) \tcp*{help operation that caused failure} \label{ISB-ll-CompleteOp-help-after-CAS}}
			\CAS (\textit{utOpInfo}$\rightarrow$pred$\rightarrow$info, \textit{OpInfo}, \textit{utOpInfo}) \tcp*{\textbf{untag} \CAS} \label{ISB-ll-CompleteOp-backtrack-CAS}
			\KwRet \False \tcp*{operation attempt failed} \label{ISB-ll-CompleteOp-return-false}
		}
	\end{procedure}


	%%%%%%%%%%%%% OP-RECOVER FUNCTION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\begin{procedure}[H]
	\color {blue} {
		\caption{() boolean \func{Op-Recover} ($\Key\ k$)}
		
		\Info\ *$\textit{OpInfo} := RD_q$ \label{ISB-ll-OpRecover-read-RDp} \;
		
		\uIf {$CP_q = 0$ or $\textit{OpInfo} = \init$} {
			Re-invoke \func{Op} \label{ISB-ll-OpRecover-first-reinvoke}
		}
		\uIf (\tcp*[f]{false response is persisted}) {$\textit{OpInfo}.result = \False$}
		{\KwRet \False \label{ISB-ll-OpRecover-return-false}}
		$test := \textit{OpInfo} \rightarrow pred \rightarrow info$ \label{ISB-ll-OpRecover-read-pred-update} \;
		\lIf {$test = GetTagged(OpInfo)$} {
			\func{CompleteOp}$(GetTagged(OpInfo))$ \tcp*[f]{operation in progress; complete it or untag} \label{ISB-ll-OpRecover-call-CompleteOp}
		}
		\lIf (\tcp*[f]{operation completed successfully}) {$\textit{OpInfo} \rightarrow result \neq \init$}
		{\KwRet $\textit{OpInfo} \rightarrow result$ \label{ISB-ll-OpRecover-return-true}}
		\lElse {
			Re-invoke \func{Op} \tcp*[f]{operation attempt failed} \label{ISB-ll-OpRecover-reinvoke}
		}
	}
	\end{procedure}

	\remove{
	%%%%%%%%%%%%% INSERT-RECOVER FUNCTIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	\begin{procedure}[H]
		\caption{() boolean \func{Insert-Recover} ($\Key\ k$)}
		
		\Info\ *$\textit{OpInfo} := RD_q$ \label{ISB-ll-InsertRecover-read-RDp} \;
		
		\uIf {$CP_q = 0$ or $\textit{OpInfo} = \init$} {
			Re-invoke \func{Insert} \label{ISB-ll-InsertRecover-first-reinvoke}
		}
		\uIf (\tcp*[f]{false response is persisted}) {$\textit{OpInfo}.result = \False$}
		{\KwRet \False \label{ISB-ll-InsertRecover-return-false}}
		$test := \textit{OpInfo}. pred. update$ \label{ISB-ll-InsertRecover-read-pred-update} \;
		\lIf {$test = \langle \mk, \textit{OpInfo} \rangle$} {
			\func{CompleteInsert}$(\textit{OpInfo})$ \tcp*[f]{insertion in progress; complete it or untag} \label{ISB-ll-InsertRecover-call-CompleteInsert}
		}
		\lIf (\tcp*[f]{insert completed successfully}) {$\textit{OpInfo}. result \neq \init$}
			{\KwRet $\textit{OpInfo}.result$ \label{ISB-ll-InsertRecover-return-true}}
		\lElse {
			Re-invoke \func{Insert} \tcp*[f]{insert attempt failed} \label{ISB-ll-InsertRecover-reinvoke}
		}
	\end{procedure}
	
	%%%%%%%%%%%%% DELETE-RECOVER FUNCTIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	\begin{procedure}[H]
		\caption{() boolean \func{Delete-Recover} ($\Key\ k$)}
		
		\Info\ *$\textit{OpInfo} = RD_q$ \label{ISB-ll-DeleteRecover-read-RDp} \;
		
		\uIf {$CP_q = 0$ or $\textit{OpInfo} = \init$} {
			Re-invoke \func{Delete} \label{ISB-ll-DeleteRecover-first-reinvoke}
		}
		\uIf (\tcp*[f]{false response is persisted}) {$\textit{OpInfo}.result = \False$}
		{\KwRet \False \label{ISB-ll-DeleteRecover-return-false}}
		$test := \textit{OpInfo}. pred. update$ \label{ISB-ll-DeleteRecover-read-pred-update} \;
		\lIf {$test = \langle \mk, \textit{OpInfo} \rangle$} {
			\func{CompleteDelete}$(\textit{OpInfo})$ \tcp*[f]{deletion in progress; complete it or untag} \label{ISB-ll-DeleteRecover-call-CompleteDelete}
		}
		\lIf (\tcp*[f]{delete completed successfully}) {$\textit{OpInfo}. result \neq \init$}
			{\KwRet $\textit{OpInfo}.result$ \label{ISB-ll-DeleteRecover-return-true}}
		\lElse {
			Re-invoke \func{Delete} \tcp*[f]{delete attempt failed} \label{ISB-ll-DeleteRecover-reinvoke}
		}
	\end{procedure}
}

	\caption{Recoverable Linked List (code for process $q$)}
%: \insertlst{}, \func{Op-Recover} \& \func{CompleteOp}}
	\label{alg:ISB-ll-recover}\label{alg:ISB-ll-insert-delete}
\end{algorithm}



==> code-exchanger-only-2col.tex <==

%%%%%%%%%%%%%%%%%%Elimination array%%%%%%%%%%%%%%%%%
\SetInd{0.25em}{0.35em}

\begin{figure*}[!t]
	\removelatexerror
	
	\begin{algorithm}[H]
		
		\begin{multicols*}{2}
		\scriptsize
		
		\begin{flushleft}
			\textcolor{blue}{
				Type \exInfo\ \{ \hspace*{24.0mm} $\triangleright$ subtype of \Info \\
				\hspace*{6mm} \{\emptyst, \waiting, \busy\} $state$ \\
				\hspace*{6mm} T $value$, $result$ \\
				\hspace*{6mm} \exInfo\ $partner$ \} \\
			}
			%	\exInfo\ $default$ - global static \exInfo\ object with state = \emptyst
			
%			\com Initialization: \\
			\textbf{Shared variables:} \\
			\hspace*{15mm} \textcolor{blue}{\exInfo\ \emph{default} := \textbf{new} \exInfo (\emptyst, \init, \init, \init)} \\
			\hspace*{15mm} \emph{ExInfo} \emph{slot}, initially \emph{default} \\
			\textbf{Private variables:} \textcolor{blue}{\Info\ $RD_q$, for each process $q$}
		\end{flushleft}
	
	
		
%		\columnbreak
		%\vspace*{-5pt}
		
		\begin{procedure}[H]
			\color{blue} {
				\caption{() \footnotesize T \recoverExchange \\
                     \hspace*{25mm} (\exInfo\ $slot$, T $value$)}
				
				\exInfo\ $myop := RD_q$ \label{ex-recover-entry} \;
				\exInfo\ $yourop := slot$ \;
		
				\lIf{$CP_q = 0$} { Re-invoke \exchange }
				
				\uIf {$myop \rightarrow state = \waiting$ \label{ex-recover-if-waiting}} {
					%\tcp{crashed while waiting}
					%$yourop := slot$ \label{exchange-recover-waiting-read-slot} \;
					\uIf (\tcp*[f]{still waiting}) {$yourop = myop$ \label{ex-recover-if-still-waiting}} {
						proceed from line \ref{ex-waiting-while} \label{ex-recover-still-waiting}
					}
					\uElseIf {$yourop \rightarrow partner = myop$ \label{ex-recover-waiting-if-collision-in-progress}} {
						\tcp{collision in progress; complete it}
						\switchPair$(myop, yourop)$ \;
						\CAS (\emph{slot}, \emph{yourop}, \emph{default}) \label{ex-recover-waiting-in-progress-release-slot}
					}
				}
				\uIf {$myop \rightarrow state = \busy$ \label{ex-recover-if-busy}} {
%					\tcp{trying to collide $myop.partner$}
					%$yourop := slot$ \label{exchange-recover-busy-read-slot} \;
					\uIf (\tcp*[f]{collision in progress}) {$yourop = myop$ \label{ex-recover-busy-collision-in-progress}} {
						%\tcp{collision in progress; complete it}
						\switchPair$(myop, myop \rightarrow partner)$ \;
						\CAS (\emph{slot}, \emph{myop}, \emph{default}) \label{ex-recover-busy-release-solt}
					}	
				}
				\uIf {$myop \rightarrow result \neq \init$ \label{ex-recover-if-persist}}
				{
					\KwRet $myop \rightarrow result$ \tcp*{operation completed} \label{ex-recover-return-persist}}
				\lElse {Re-invoke \exchange} \label{ex-recover-reinvoke}
			}
		\end{procedure}
	
		\begin{procedure}[H]
			\color{blue}{
				\caption{() \footnotesize void \switchPair \\
					\hspace*{22mm} (\exInfo\ $first$, \exInfo\ $second$)}
				
				\tcp{exchange values of two operations}
				\emph{first} $\rightarrow$ \emph{result} := \emph{second} $\rightarrow$ \emph{value} \;
				\emph{second} $\rightarrow$ \emph{result} := \emph{first} $\rightarrow$ \emph{value} \;
			}
		\end{procedure}
	
		\columnbreak
		
				
		\begin{procedure}[H]
			\caption{() \small T \exchange \\
				\hspace*{25mm} (\exInfo\ $slot$, T $value$)}
			
			\textcolor{blue}{\exInfo\ $myop$ := \textbf{new} \exInfo
				(\waiting, $value$, \init, \init)} \label{ex-new-info} \;
			\textcolor{blue}{$RD_q$ := $myop$} \tcp*{set Info structure} \label{ex-update-RD}
			\textcolor{blue}{$CP_q := 1$} \tcp*{set a check-point} \label{ex-set-checkpoint}
			
			\While{\True \label{ex-outer-while}} {
				$yourop := slot$ \label{ex-read-slot} \;
				%		$\langle$youritem,state$\rangle$ := slot\;
				\Switch{$yourop \rightarrow state$} {
					\uCase (\tcp*[f]{try to capture exchanger}) {\emptyst \label{ex-case-empty}} {
						\textcolor{blue}{$myop \rightarrow state$ := \waiting} \label{ex-waiting-set-state} \;
						\textcolor{blue}{$myop \rightarrow partner := \init$} \label{ex-waiting-reset-partner} \;
						\If {$\CAS (slot, yourop, myop)$ \label{ex-waiting-cas}} {
							\While {\True \label{ex-waiting-while}} {
								$yourop := slot$ \tcp*{check for collision} \label{ex-waiting-read-slot}
								\uIf {$yourop \neq myop$ \label{ex-waiting-collision-detect}} {
									\uIf {\textcolor{blue}{$yourop \rightarrow partner = myop$} \label{ex-waiting-if-collision-in-progress}} {
										\tcp{collision is in progress}
										\textcolor{blue}{\switchPair $(myop, yourop)$} \label{ex-waiting-complete-collision} \;
										\textcolor{blue}{\CAS (\emph{slot}, \emph{yourop}, \emph{default})} \label{ex-waiting-reset-slot}
									}
									\KwRet $myop \rightarrow result$ \label{ex-waiting-return} \; } } }
						break \;
					}
					\uCase (\tcp*[f]{try to collide}) {\waiting \label{ex-case-waiting}} {
						\textcolor{blue}{$myop \rightarrow partner := yourop$} \label{ex-busy-set-partner} \;
						\textcolor{blue}{$myop \rightarrow state := \busy$} \tcp*{announce - attempting to collide with $yourop$} \label{ex-busy-set-state}
						\uIf {$\CAS (slot, yourop, myop)$ \label{ex-busy-cas}} {
							\textcolor{blue}{\switchPair $(myop, yourop)$} \label{ex-busy-complete-collision} \;
							\textcolor{blue}{\CAS (\emph{slot}, \emph{myop}, \emph{default})} \label{ex-busy-reset-slot} \;
							\KwRet $myop \rightarrow result$ \label{ex-busy-return-response} \;
						}
						break \;
					}
					\uCase (\tcp*[f]{a collision in progress}) {\busy \label{ex-case-busy}} {
						\textcolor{blue}{\switchPair $(yourop, yourop \rightarrow partner)$} \label{ex-occupied-complete-collision} \;
						\textcolor{blue}{\CAS (\emph{slot}, \emph{yourop}, \emph{default})} \label{ex-occupied-release-slot} \;
						break \;
					}
				}	
			}
		\end{procedure}
	
		
	\end{multicols*}

		\caption{Recoverable Exchanger (process $q$)}
		\label{alg:exchanger}
	\end{algorithm}
	
\end{figure*}


==> code-exchanger-only.tex <==

%%%%%%%%%%%%%%%%%%Elimination array%%%%%%%%%%%%%%%%%
\SetInd{0.25em}{0.35em}

\begin{figure}[!t]
	\removelatexerror
	
	\begin{algorithm}[H]
		
%		\begin{multicols*}{2}
		\scriptsize
		
		\begin{flushleft}
			\textcolor{blue}{
				Type \exInfo\ \{ \hspace*{24.0mm} $\triangleright$ subtype of \Info \\
				\hspace*{6mm} \{\emptyst, \waiting, \busy\} $state$ \\
				\hspace*{6mm} T $value$, $result$ \\
				\hspace*{6mm} \exInfo\ $partner$ \\
				\}
			}
			%	\exInfo\ $default$ - global static \exInfo\ object with state = \emptyst
			
%			\com Initialization: \\
			\textbf{Shared variables:} \textcolor{blue}{\exInfo\ \emph{default} := \textbf{new} \exInfo (\emptyst, \init, \init, \init)} \\
			\hspace*{21mm} \emph{ExInfo} \emph{slot}, initially \emph{default} \\
			\textbf{Private variables:} \textcolor{blue}{\Info\ $RD_q$, for each process $q$}
		\end{flushleft}
	
	
		
%		\columnbreak
		
		\begin{procedure}[H]
			\caption{() \small T \exchange
				\hspace*{5mm} (\exInfo\ $slot$, T $value$)}
			
			\textcolor{blue}{\exInfo\ $myop$ := \textbf{new} \exInfo
				(\waiting, $value$, \init, \init)} \label{ex-new-info} \;
			\textcolor{blue}{$RD_q$ := $myop$} \tcp*{set Info structure} \label{ex-update-RD}
			\textcolor{blue}{$CP_q := 1$} \tcp*{set a check-point} \label{ex-set-checkpoint}
			
			\While{\True \label{ex-outer-while}} {
				$yourop := slot$ \label{ex-read-slot} \;
				%		$\langle$youritem,state$\rangle$ := slot\;
				\Switch{$yourop.state$} {
					\uCase (\tcp*[f]{try to capture exchanger}) {\emptyst \label{ex-case-empty}} {
						\textcolor{blue}{$myop.state$ := \waiting} \label{ex-waiting-set-state} \;
						\textcolor{blue}{$myop.partner := \init$} \label{ex-waiting-reset-partner} \;
						\If {$\CAS (slot, yourop, myop)$ \label{ex-waiting-cas}} {
							\While {\True \label{ex-waiting-while}} {
								$yourop := slot$ \tcp*{check for collision} \label{ex-waiting-read-slot}
								\uIf {$yourop \neq myop$ \label{ex-waiting-collision-detect}} {
									\uIf {\textcolor{blue}{$yourop.partner = myop$} \label{ex-waiting-if-collision-in-progress}} {
										\tcp{collision is in progress}
										\textcolor{blue}{\switchPair $(myop, yourop)$} \label{ex-waiting-complete-collision} \;
										\textcolor{blue}{\CAS (\emph{slot}, \emph{yourop}, \emph{default})} \label{ex-waiting-reset-slot}
									}
									\KwRet $myop.result$ \label{ex-waiting-return} \; } } }
						break \;
					}
					\uCase (\tcp*[f]{try to collide}) {\waiting \label{ex-case-waiting}} {
						\textcolor{blue}{$myop.partner := yourop$} \label{ex-busy-set-partner} \;
						\textcolor{blue}{$myop.state := \busy$} \tcp*{announce - attempting to collide with $yourop$} \label{ex-busy-set-state}
						\uIf {$\CAS (slot, yourop, myop)$ \label{ex-busy-cas}} {
							\textcolor{blue}{\switchPair $(myop, yourop)$} \label{ex-busy-complete-collision} \;
							\textcolor{blue}{\CAS (\emph{slot}, \emph{myop}, \emph{default})} \label{ex-busy-reset-slot} \;
							\KwRet $myop.result$ \label{ex-busy-return-response} \;
						}
						break \;
					}
					\uCase (\tcp*[f]{a collision in progress}) {\busy \label{ex-case-busy}} {
						\textcolor{blue}{\switchPair $(yourop, yourop.partner)$} \label{ex-occupied-complete-collision} \;
						\textcolor{blue}{\CAS (\emph{slot}, \emph{yourop}, \emph{default})} \label{ex-occupied-release-slot} \;
						break \;
					}
				}	
			}
		\end{procedure}
		
		
		\begin{procedure}[H]
			\color{blue} {
				\caption{() \small T \recoverExchange
                    (\exInfo\ $slot$, T $value$)}
				
				\exInfo\ $myop := RD_q$ \label{ex-recover-entry} \;
				\exInfo\ $yourop := slot$ \;
		
				\lIf{$CP_q = 0$} { Re-invoke \exchange }
				
				\uIf {$myop.state = \waiting$ \label{ex-recover-if-waiting}} {
					%\tcp{crashed while waiting}
					%$yourop := slot$ \label{exchange-recover-waiting-read-slot} \;
					\uIf (\tcp*[f]{still waiting}) {$yourop = myop$ \label{ex-recover-if-still-waiting}} {
						proceed from line \ref{ex-waiting-while} \label{ex-recover-still-waiting}
					}
					\uElseIf {$yourop.partner = myop$ \label{ex-recover-waiting-if-collision-in-progress}} {
						\tcp{collision in progress; complete it}
						\switchPair$(myop, yourop)$ \;
						\CAS (\emph{slot}, \emph{yourop}, \emph{default}) \label{ex-recover-waiting-in-progress-release-slot}
					}
				}
				\uIf {$myop.state = \busy$ \label{ex-recover-if-busy}} {
%					\tcp{trying to collide $myop.partner$}
					%$yourop := slot$ \label{exchange-recover-busy-read-slot} \;
					\uIf {$yourop = myop$ \label{ex-recover-busy-collision-in-progress}} {
						\tcp{collision in progress; complete it}
						\switchPair$(myop, myop.partner)$ \;
						\CAS (\emph{slot}, \emph{myop}, \emph{default}) \label{ex-recover-busy-release-solt}
					}	
				}
				\uIf {$myop.result \neq \init$ \label{ex-recover-if-persist}}
				{
					\KwRet $myop.result$ \tcp*{operation completed} \label{ex-recover-return-persist}}
				\lElse {Re-invoke \exchange} \label{ex-recover-reinvoke}
			}
		\end{procedure}
	
		\begin{procedure}[H]
			\color{blue}{
				\caption{() \small void \switchPair
					(\exInfo\ $first$, \exInfo\ $second$)}
				
				\tcp{exchange values of two operations}
				\emph{first}.\emph{result} := \emph{second}.\emph{value} \;
				\emph{second}.\emph{result} := \emph{first}.\emph{value} \;
			}
		\end{procedure}
		
%	\end{multicols*}

		\caption{Recoverable Exchanger (process $q$)}
		\label{alg:exchanger}
	\end{algorithm}
	
\end{figure}


==> code-flush-linked-list.tex <==
\newcommand{\flushes}[1]{{\color{orange} #1}\normalcolor}
\newcommand{\initlist}{\mbox{\sc InitList}}
\newcommand{\flush}{\mbox{\sc FLUSH}}


%\setlength{\columnsep}{-0.1cm}

\SetInd{0.25em}{0.5em}

\begin{figure}[!h]
	\removelatexerror
	
%	\hspace*{-0.3in}
	\begin{algorithm}[H]
		
		
		\begin{multicols*}{2}
		\scriptsize
			
		\begin{flushleft}		
			\begin{tabular}{ll}
				\textbf{Type} Node & \{MarkableNodeRef $next$, int \emph{key}, \textcolor{blue} {int \emph{deleter}}, \\ 
				& \flushes{boolean \emph{flushed}}\} \\
				\textcolor{blue}{\textbf{Type} \Info} & \textcolor{blue} {\{Node $nd$, boolean $result$\}}\\
			\end{tabular}
			\textbf{Shared variables:} Node $head$ \\
			\textbf{Private variables:} \textcolor{blue} {$\Info\ RD_p$ for each process p}
		\end{flushleft}	
			
		%%%%%%%%%%%%%%%%%%%%%% Flush Linked List - Init %%%%%%%%%%%%%%%%%%%%%%%%
		\begin{procedure}[H]
			\flushes{\caption{() \small Node \initlist\ ()}}
			\flushes{Node $head :=$ \textbf{new} Node ($\bot, INT\_MIN, \init, \True$)} \label{flush-ll-init-start} \;
			\flushes{\flush($head$)} \;
			\flushes{$head.next :=$ \textbf{new} Node ($\bot, INT\_MAX, \init, \True$)}\;
			\flushes{\flush($head.next$)} \;
			\flushes{\KwRet $head$} \label{flush-ll-init-end}
		\end{procedure}



		%%%%%%%%%%%%%%%%%%%%%% Linked List - Find %%%%%%%%%%%%%%%%%%%%%%%%
		\begin{procedure}[H]
			\caption{() \small boolean \find\ (T $key$)}
			
			Node $curr$, \flushes{$succ$} \label{flush-ll-find-start} \;
			$curr$ := $head$\;
			\tcp{search for first node with key $\geq$ $key$}
			\While {$curr.key < key$}{
				\flushes{$succ := unmark(curr.next)$}\;	\label{flush-ll-find-read-succ}
				\uIf{\flushes{$succ.flushed = \False$}} {
					\flushes{\flush($curr.next$)}\;
					\flushes{$succ.flushed := \True$}\;
					\flushes{\flush($succ.flushed$)}\;
				}
				\flushes{$curr := succ$}\;	\label{flush-ll-find-update-curr}	
			}
			\KwRet ($curr.key = key\ \&\&\ \neg ismarked(curr.next)$) \label{flush-ll-find-end}
		\end{procedure}		
		
		\columnbreak		
		
		%%%%%%%%%%%%%%%%%%%%%% Linked List - Search %%%%%%%%%%%%%%%%%%%%%%%%
		
		\begin{procedure}[H]
			\caption{() \small $\langle$Node, Node$\rangle$ \search\ (T $key$)}
			
			Node $pred$, $curr$, $succ$ \;
			\textbf{retry:} \label{flush-ll-search-outer-loop}
				$pred := head$ \;
				\hspace*{7mm} $curr := pred.next$ \label{flush-ll-search-read-cur}\;	
				\While{\True}{
					$succ := curr.next$ \;
					\tcp{if $curr$ was logically deleted}
					\uIf {$ismarked(succ)$} {
						\uIf (\tcp*[f]{help delete}) {$\CAS (pred.next, curr$, $unmark(succ)$) = \False}{
							\textbf{go to} retry \tcp*{help failed}
						}
						$curr := unmark(succ)$ \tcp*{help succeeded}
					} \uElse {
						\uIf{\flushes{$curr.flushed = \False$}} {
							\flushes{\flush($pred.next$)}\;
							\flushes{$curr.flushed := \True$}\;
							\flushes{\flush($curr.flushed$)}
						}		
						
						\uIf (\tcp*[f]{first unmarked node with key $\geq key$}) {$curr.key \geq key$} {
							\KwRet $\langle pred,curr \rangle$
						}
						$pred := curr$ \tcp*{advance $pred$}
						$curr := succ$ \tcp*{advance $curr$}
					}
				}
		\end{procedure}	

		\end{multicols*}
		
		\caption{Recoverable Linked List with flushes: \initlist, \find, and \search} \label{alg:flush-ll-1}
	\end{algorithm}

	
\end{figure}
	


\begin{figure}[!t]
	\removelatexerror
	
%	\hspace*{-0.3in}
	\begin{algorithm}[H]
		
		
		\begin{multicols*}{2}
		\scriptsize
		\begin{flushleft}	
		\end{flushleft}
		\vspace{-6.5mm}
	
		%%%%%%%%%%%%% Recoverable Linked List - Delete %%%%%%%%%%%%%%%%%%%
		
		\begin{procedure}[H]
			\caption{() \small boolean \delete\ (T $key$)}
			
			Node $pred$, $curr$, $succ$  \;
			boolean $res$ := \False \;
			\textcolor{blue} {$RD_p$ := \textbf{new} \Info\ (\init, \init) \tcp*{set \Info\ structure}} \label{flush-ll-delete-persist-to-RDp}
			\flushes{\flush($RD_p$)}\;
			\textcolor{blue} {$CP_p := 1$ \tcp*{set a check-point} \label{flush-ll-delete-set-checkpoint}}
			\flushes{\flush($CP_p$)}\;
			$\langle pred, curr \rangle := \search (key)$ \tcp*{search for $key$} \label{flush-ll-search-in-delete}
			\uIf (\tcp*[f]{$key$ not in the list}) {$curr.key \neq key$ \label{flush-ll-delete-key-in-list}} {
				\textcolor{blue} {$RD_p.result := \False$ \tcp*{persist response}} \label{flush-ll-delete-write-false}
				\flushes{\flush($RD_p.result$)}\;				
				\KwRet \False \label{flush-ll-delete-return-false}
			}
			\uElse {
				\textcolor{blue}{$RD_p.nd := curr$ \tcp*{persist curr reference}} \label{flush-ll-delete-update-nd}
				\flushes{\flush($RD_p.nd$)}\;
				\While {$\lnot ismarked(curr.next)$  \label{flush-ll-delete-while-loop}}{
					\tcp{repeatedly attempt logical delete}
					$succ := curr.next$ \label{flush-ll-delete-set-succ-to-next}\;
					\uIf {\CAS ($curr.next$, $unmark(succ)$, $mark(succ)$)}{ \label{flush-ll-delete-logical-delete}
						\flushes{\flush($curr.next$)}
					}
				}
				\tcp{Physical deletion attempt}
				$succ := curr.next$ \label{flush-ll-delete-read-succ-after-CAS}\;
				\CAS ($pred.next$, $curr$, $unmark(succ)$) \label{flush-ll-delete-physical-delete} \;
				\textcolor{blue}{\tcp{try establishing yourself as deleter}}
				\textcolor{blue}{$res := \CAS (curr.deleter, \init, p)$}  \label{flush-ll-delete-CAS-deleter} \;
				\flushes{\flush($curr.deleter$)}\;
				\textcolor{blue}{$RD_p.result := res$ \tcp*{persist response}} \label{flush-ll-delete-write-after-CAS}
				\flushes{\flush($RD_p.result$)}\;				
				\KwRet $res$ \label{flush-ll-delete-return-res}
			}		
		\end{procedure}
		
		%%%%%%%%%%%%% Recoverable Linked List - Delete Recover %%%%%%%%%%%%
	
	\textcolor{blue}{
		\begin{procedure}[H]
			\caption{() \small \text{boolean \deleterecover\ (T $key$)}}
			Node $nd$ := $RD_p.nd$ \;
			boolean $res$ := \False \;
			\uIf {$CP_p = 0$ \label{flush-ll-delete-recover-read-CP}} {
				\tcc{failed before check-point}
				Re-invoke \delete
			}
			\uIf {$RD_p.result \neq \init$ \label{flush-ll-delete-recover-response-persisted}} {
				\tcc{operation response was persisted}
				\KwRet $RD_p.result$ \label{flush-ll-delete-recover-return-persisted-response}
			}
			\uIf {$nd \neq \init$ \&\& $ismarked(nd.next)$ \label{flush-ll-delete-recover-if-should-perform-deleter-CAS}} {
				\tcc{$nd$ was logically deleted; try establish yourself as deleter}
				$\CAS (nd.deleter, \init, p)$ \label{flush-ll-delete-recover-deleter-CAS} \;
				\flushes{\flush($nd.deleter$)} \textcolor{blue}{ \; 
				$res := (nd.deleter == p)$ \label{flush-ll-delete-recover-read-deleter} \;
				$RD_p.result := res$ \tcp*{persist response}}
				\flushes{\flush($RD_p.result$)} \textcolor{blue}{ \;
				\KwRet res \label{flush-ll-delete-recover-return-res}\;}
			}
			\lElse {
				Re-invoke \delete \label{flush-ll-delete-recover-reattempt-deletion} \tcp*[f]{re-attempt deletion}
			}
		\end{procedure}
	}
		\columnbreak
	
		%%%%%%%%%%%%%% Recoverable Linked List - Insert %%%%%%%%%%%%%%%%%
			
		\begin{procedure}[H]
			\caption{() \small boolean \insertlst\ (T $key$)}
			
			Node $pred$, $curr$, $newnd$ := \textbf{new} Node ($\init, key, \textcolor{blue}{\init}, \flushes{\False}$) \label{flush-ll-insert-entry} \;
			%Node $newnd$ := \textbf{new} Node ($\init, key, \textcolor{blue}{\init}$)\;
			%\textcolor{blue}{newnd.deleter := \init} \;
			\textcolor{blue} {$RD_p$ := \textbf{new} \Info\ ($newnd$, \init) \label{flush-ll-insert-install-IS}} \;
			\flushes{\flush($RD_p$)}\;
			\textcolor{blue} {$\text{CP}_p := 1$ \tcp*{set a check-point}\label{flush-ll-insert-set-checkpoint}}
			\flushes{\flush($CP_p$)}\;
			\While{\True}{ \label{flush-ll-insert-while}
				\tcp{search for right location to insert}
				$\langle pred, curr \rangle := \search(key)$ \label{flush-ll-insert-search} \;
				\uIf (\tcp*[f]{$key$ in the list}) {$curr.key = key$ \label{flush-ll-insert-if-in-list}} {
					\textcolor{blue} {$RD_p.result := \False$ \tcp*{persist response} \label{flush-ll-insert-persist-false-response}}
					\flushes{\flush($RD_p.result$)}\;
					\KwRet \False \label{flush-ll-insert-return-false}
				} \uElse {
					$newnd.next$ := $curr$\;
					\uIf (\tcp*[f]{try to add $newnd$}) {\CAS ($pred.next$, $curr$, $newnd$) \label{flush-ll-insert-CAS}} {
						\flushes{\flush($pred.next$)}\;
						\flushes{$newnd.flushed := \True$}\;
						\flushes{\flush($newnd.flushed$)}\;
						\textcolor{blue} {$RD_p.result := \True$ \label{flush-ll-insert-persist-true-response}} \;
						\flushes{\flush($RD_p.result$)}\;
						\KwRet \True
					}
				}		
			}
		\end{procedure}


		
		
		%%%%%%%%%%%%% Recoverable Linked List - Insert Recover %%%%%%%%%%
	
	\textcolor{blue}{
		\begin{procedure}[H]
			\caption{() \small \text{boolean \insertrecover\ (T $key$)}}
			%
			Node $nd := RD_p.nd$\;
			\uIf {$CP_p := 0$ \label{flush-ll-insert-recover-read-CP}} {
				\tcc{failed before check-point}		
				Re-invoke \insertlst \label{flush-ll-insert-recover-re-invoke}
			}
			\uIf {$RD_p.result \neq \init$ \label{flush-ll-insert-recover-response-persisted}} {
				\tcc{operation response was persisted}
				\KwRet $RD_p.result$ \tcp*[f]{return response \label{flush-ll-insert-recover-return-persisted-response}}
			}
			$\langle pred, curr \rangle := \search (key)$ \label{flush-ll-insert-recover-search} \;
			\uIf {$curr = nd \mid \mid ismarked(nd.next)$ \label{flush-ll-insert-if-was-linearized}} {
				\tcp{$nd$ in list or is marked (hence was)}
				$RD_p.result := \True$ \tcp*{persist response} \label{flush-ll-insert-linearized-persist-true}
				\flushes{\flush($RD_p.result$)} \textcolor{blue}{ \;
				\KwRet \True \label{flush-ll-insert-linearized-return-true}\;}
			}
			\lElse
			{
				Re-invoke \insertlst \tcp*[f]{re-attempt insertion}
			}
		\end{procedure}
	}
	
	
	\end{multicols*}
		
		\caption{Recoverable Linked List with flushes: \delete, \deleterecover, \insertlst, and \insertrecover} \label{alg:flush-ll-2}
	\end{algorithm}

	
\end{figure}

==> code-linked-list.tex <==
%\setlength{\columnsep}{-0.1cm}

\SetInd{0.25em}{0.5em}

\begin{figure}[!t]
	\removelatexerror
	
%	\hspace*{-0.3in}
	\begin{algorithm}[H]
		
		
		\begin{multicols*}{2}
		\scriptsize
			
		\begin{flushleft}
			
			\begin{tabular}{ll}
				\textbf{Type} Node & \{MarkableNodeRef $next$, int \emph{key}, \textcolor{blue} {int \emph{deleter}}\} \\
				\textcolor{blue}{\textbf{Type} \Info} & \textcolor{blue} {\{Node $nd$, boolean $result$\}}\\
			\end{tabular}
			\textbf{Shared variables:} Node $head$ \\
			\textbf{Private variables:} \textcolor{blue} {$\Info\ RD_p$ for each process p}
		\end{flushleft}	
			
		
		%%%%%%%%%%%%%%%%%%%%%% Linked List - Find %%%%%%%%%%%%%%%%%%%%%%%%
		\begin{procedure}[H]
			\caption{() \small Boolean \find\ (T $key$)}
			
			Node $curr$ := $head$ \label{ll-find-start} \;
			\tcp{search for first node with key $\geq$ $key$}
			\While {$curr.key < key$}{
				$curr := curr.next$ \label{ll-find-read-cur}\;	
			}
			\KwRet ($curr.key = key\ \&\&\ \neg ismarked(curr.next)$) \label{ll-find-end}
		\end{procedure}
	
	
		%%%%%%%%%%%%% Recoverable Linked List - Delete %%%%%%%%%%%%%%%%%%%
		
		\begin{procedure}[H]
			\caption{() \small Boolean \delete\ (T $key$)}
			
			Node $pred$, $curr$, $succ$  \;
			boolean $res$ := \False \;
			\textcolor{blue} {$RD_p$ := \textbf{new} \Info\ (\init, \init) \tcp*{set \Info\ structure}} \label{ll-delete-persist-to-RDp}
			\textcolor{blue} {$CP_p := 1$ \tcp*{set a check-point} \label{ll-delete-set-checkpoint}}
			$\langle pred, curr \rangle := \search (key)$ \tcp*{search for $key$} \label{ll-search-in-delete}
			\uIf (\tcp*[f]{$key$ not in the list}) {$curr.key \neq key$ \label{ll-delete-key-in-list}} {
				\textcolor{blue} {$RD_p.result := \False$ \tcp*{persist response}} \label{ll-delete-write-false}
				\KwRet \False \label{ll-delete-return-false}
			}
			\uElse {
				\textcolor{blue}{$RD_p.nd := curr$ \tcp*{persist curr reference}} \label{ll-delete-update-nd}
				\While {$\lnot ismarked(curr.next)$  \label{ll-delete-while-loop}}{
					\tcp{repeatedly attempt logical delete}
					$succ := curr.next$ \label{ll-delete-set-succ-to-next}\;
					\CAS ($curr.next$, $unmark(succ)$, $mark(succ)$) \label{ll-delete-logical-delete}\;
				}
				\tcp{Physical deletion attempt}
				$succ := curr.next$ \label{ll-delete-read-succ-after-CAS}\;
				\CAS ($pred.next$, $curr$, $unmark(succ)$) \label{ll-delete-physical-delete} \;
				\textcolor{blue}{\tcp{try establishing yourself as deleter}}
				\textcolor{blue}{$res := \CAS (curr.deleter, \init, p)$}  \label{ll-delete-CAS-deleter} \;
				\textcolor{blue}{$RD_p.result := res$ \tcp*{persist response}} \label{ll-delete-write-after-CAS}
				\KwRet $res$ \label{ll-delete-return-res}
			}		
		\end{procedure}
	
		%%%%%%%%%%%%%% Recoverable Linked List - Insert %%%%%%%%%%%%%%%%%
		
		\begin{procedure}[H]
			\caption{() \small Boolean \insertlst\ (T $key$)}
			
			Node $pred$, $curr$, $newnd$ := \textbf{new} Node ($\init, key, \textcolor{blue}{\init}$) \label{ll-insert-entry} \;
			%Node $newnd$ := \textbf{new} Node ($\init, key, \textcolor{blue}{\init}$)\;
			%\textcolor{blue}{newnd.deleter := \init} \;
			\textcolor{blue} {$RD_p$ := \textbf{new} \Info\ ($newnd$, \init) \label{ll-insert-install-IS}} \;
			\textcolor{blue} {$\text{CP}_p := 1$ \tcp*{set a check-point}\label{ll-insert-set-checkpoint}}
			\While{\True}{ \label{ll-insert-while}
				\tcp{search for right location to insert}
				$\langle pred, curr \rangle := \search(key)$ \label{ll-insert-search} \;
				\uIf (\tcp*[f]{$key$ in the list}) {$curr.key = key$ \label{ll-insert-if-in-list}} {
					\textcolor{blue} {$RD_p.result := \False$ \tcp*{persist response} \label{ll-insert-persist-false-response}}
					\KwRet \False \label{ll-insert-return-false}
				} \uElse {
					$newnd.next$ := $curr$\;
					\uIf (\tcp*[f]{try to add $newnd$}) {\CAS ($pred.next$, $curr$, $newnd$) \label{ll-insert-CAS}} {
						\textcolor{blue} {$RD_p.result := \True$ \label{ll-insert-persist-true-response}} \;
						\KwRet \True
					}
				}		
			}
		\end{procedure}
		
		\columnbreak
		
		%%%%%%%%%%%%%%%%%%%%%% Linked List - Search %%%%%%%%%%%%%%%%%%%%%%%%
		
		\begin{procedure}[H]
			\caption{() \small $\langle$Node, Node$\rangle$ \search\ (T $key$)}
			
			Node $pred$, $curr$, $succ$ \;
			\textbf{retry:} \label{ll-search-outer-loop}
				$pred := head$ \;
				\hspace*{7mm} $curr := pred.next$ \label{ll-search-read-cur}\;	
				\While{\True}{
					$succ := curr.next$ \;
					\tcp{if $curr$ was logically deleted}
					\uIf {$ismarked(succ)$} {
						\uIf (\tcp*[f]{help delete}) {$\CAS (pred.next, curr$, $unmark(succ)$) = \False}{
							\textbf{go to} retry \tcp*{help failed}
						}
						$curr := unmark(succ)$ \tcp*{help succeeded}
					} \uElse {
						\uIf (\tcp*[f]{first unmarked node with key $\geq key$}) {$curr.key \geq key$} {
							\KwRet $\langle pred,curr \rangle$
						}
						$pred := curr$ \tcp*{advance $pred$}
						$curr := succ$ \tcp*{advance $curr$}
					}
				}
		\end{procedure}
	
	
	%%%%%%%%%%%%% Recoverable Linked List - Delete Recover %%%%%%%%%%%%
	
	\textcolor{blue}{
		\begin{procedure}[H]
			\caption{() \small \text{Boolean \deleterecover\ (T $key$)}}
			Node $nd$ := $RD_p.nd$ \;
			boolean $res$ := \False \;
			\uIf {$CP_p = 0$ \label{ll-delete-recover-read-CP}} {
				\tcc{failed before check-point}
				Re-invoke \delete
			}
			\uIf {$RD_p.result \neq \init$ \label{ll-delete-recover-response-persisted}} {
				\tcc{operation response was persisted}
				\KwRet $RD_p.result$ \label{ll-delete-recover-return-persisted-response}
			}
			\uIf {$nd \neq \init$ \&\& $ismarked(nd.next)$ \label{ll-delete-recover-if-should-perform-deleter-CAS}} {
				\tcc{$nd$ was logically deleted; try establish yourself as deleter}
				$\CAS (nd.deleter, \init, p)$ \label{ll-delete-recover-deleter-CAS} \;
				$res := (nd.deleter == p)$ \label{ll-delete-recover-read-deleter} \;
				$RD_p.result := res$ \tcp*{persist response}
				\KwRet res \label{ll-delete-recover-return-res}\;
			}
			\lElse {
				Re-invoke \delete \label{ll-delete-recover-reattempt-deletion} \tcp*[f]{re-attempt deletion}
			}
		\end{procedure}
	}
	
	%%%%%%%%%%%%% Recoverable Linked List - Insert Recover %%%%%%%%%%
	
	\textcolor{blue}{
		\begin{procedure}[H]
			\caption{() \small \text{Boolean \insertrecover\ (T $key$)}}
			%
			Node $nd := RD_p.nd$\;
			\uIf {$CP_p := 0$ \label{ll-insert-recover-read-CP}} {
				\tcc{failed before check-point}		
				Re-invoke \insertlst \label{ll-insert-recover-re-invoke}
			}
			\uIf {$RD_p.result \neq \init$ \label{ll-insert-recover-response-persisted}} {
				\tcc{operation response was persisted}
				\KwRet $RD_p.result$ \tcp*[f]{return response \label{ll-insert-recover-return-persisted-response}}
			}
			$\langle pred, curr \rangle := \search (key)$ \label{ll-insert-recover-search} \;
			\uIf {$curr = nd \mid \mid ismarked(nd.next)$ \label{ll-insert-if-was-linearized}} {
				\tcp{$nd$ in list or is marked (hence was)}
				$RD_p.result := \True$ \tcp*{persist response} \label{ll-insert-linearized-persist-true}
				\KwRet \True \label{ll-insert-linearized-return-true}\;
			}
			\lElse
			{
				Re-invoke \insertlst \tcp*[f]{re-attempt insertion}
			}
		\end{procedure}
	}
	
	\end{multicols*}
		
		\caption{Recoverable Linked List; some implementation details follow~\cite{DBLP:books/daglib/0020056}.} \label{alg:ll}
	\end{algorithm}

	
\end{figure} 
